Differentially Private Online Learning

In this paper, we consider the problem of preserving privacy in the online learning setting. We study the problem in the online convex programming (OCP) framework---a popular online learning setting with several interesting theoretical and practical implications---while using differential privacy as the formal privacy measure. For this problem, we distill two critical attributes that a private OCP algorithm should have in order to provide reasonable privacy as well as utility guarantees: 1) linearly decreasing sensitivity, i.e., as new data points arrive their effect on the learning model decreases, 2) sub-linear regret bound---regret bound is a popular goodness/utility measure of an online learning algorithm. Given an OCP algorithm that satisfies these two conditions, we provide a general framework to convert the given algorithm into a privacy preserving OCP algorithm with good (sub-linear) regret. We then illustrate our approach by converting two popular online learning algorithms into their differentially private variants while guaranteeing sub-linear regret ($O(\sqrt{T})$). Next, we consider the special case of online linear regression problems, a practically important class of online learning problems, for which we generalize an approach by Dwork et al. to provide a differentially private algorithm with just $O(\log^{1.5} T)$ regret. Finally, we show that our online learning framework can be used to provide differentially private algorithms for offline learning as well. For the offline learning problem, our approach obtains better error bounds as well as can handle larger class of problems than the existing state-of-the-art methods Chaudhuri et al.

==> IGD.tex <==
\subsection{ Sensitivity of IGD Algorithm} 
\label{sec:IGDSensitive} 

We present the proof of the bound on the sensitivity of our \igd\ algorithm here. 

\begin{lemma}[{\bf \igd\ Sensitivity}]
Sensitivity of the \igd\ algorithm is $\frac{2L}{t}$ for the $t$-th iterate, where $L$ is the maximum Lipschitz constant of any function $f_{\tau}, 1\leq \tau\leq t$. 
\label{lem:Sen}
\end{lemma}
\begin{proof}
We prove the above lemma using mathematical induction. \\
{\bf Base Case ($t=1$)}: As $\x_1$ is selected randomly, it's value doesn't depend on the underlying dataset. \\
{\bf Induction Step $t=\tau+1$}: As $f_\tau$ is $\alpha$ strongly convex. The total convexity of the function $$\tilde{f}_\tau(\x)=\frac{1}{2}\|\x-\x_{\tau}\|_2^2+\eta_\tau f_\tau(\x),$$ 
is $\frac{\tau+1}{\tau}$. Now using strong convexity and the fact that at optima $\x_{\tau+1}$,
$$\partial \tilde{f}_\tau(\x_{\tau+1}) (\x-\x_{\tau+1})\geq 0, \forall \x\in \C,$$
we get:
\begin{equation}
  \label{eq:sens_opt_r}
  \tilde{f}_\tau(\x_{\tau+1}')\geq \tilde{f}_\tau(\x_{\tau+1})+\frac{\tau+1}{2\tau}\|\x_{\tau+1}-\x_{\tau+1}'\|_2^2.
\end{equation}
Now, we consider two cases:
\begin{itemize}
\item {\bf $F-F'=\{f_\tau\}$}: Define $\tilde{f}_\tau'(\x)=\frac{1}{2}\|\x-\x_{\tau}\|^2+\eta_\tau f_\tau'(\x)$ and let $\x_{\tau+1}'=\argmin_{\x\in \C} \tilde{f}_\tau'(\x)$. Then, similar to \eqref{eq:sens_opt_r}, we get:
\begin{equation}
  \label{eq:sens_opt_rp1}
  \tilde{f}_\tau'(\x_{\tau+1})\geq \tilde{f}_\tau'(\x_{\tau+1}')+\frac{\tau+1}{2\tau}\|\x_{\tau+1}-\x_{\tau+1}'\|_2^2.
\end{equation}
Adding \eqref{eq:sens_opt_r} and \eqref{eq:sens_opt_rp1}, we get:
$$\|\x_{\tau+1}-\x_{\tau+1}'\|_2^2\leq \frac{1}{\tau+1}|f_\tau(\x_{\tau+1}')+f_\tau'(\x_{\tau+1})-f_\tau(\x_{\tau+1})-f_\tau'(\x_{\tau+1}')|\leq \frac{2L}{\tau+1}\|\x_{\tau+1}-\x_{\tau+1}'\|_2.$$
Lemma now follows using simplification. 
\item {\bf $F-F'=\{f_i\},\ i<\tau$}: Define $\tilde{f}_\tau'(\x)=\frac{1}{2}\|\x-\x_\tau'\|^2+\eta_\tau f_\tau(\x)$ and let $\x_{\tau+1}'=\argmin_{\x\in \C} \tilde{f}_\tau'(\x)$. Then, similar to \eqref{eq:sens_opt_r}, we get:
\begin{equation}
  \label{eq:sens_opt_rp11}
  \tilde{f}_\tau'(\x_{\tau+1})\geq \tilde{f}_\tau'(\x_{\tau+1}')+\frac{\tau+1}{2\tau}\|\x_{\tau+1}-\x_{\tau+1}'\|_2^2.
\end{equation}
Adding \eqref{eq:sens_opt_r} and \eqref{eq:sens_opt_rp11}, we get:
$$\|\x_{\tau+1}-\x_{\tau+1}'\|_2^2\leq \frac{\tau}{\tau+1}|(\x_{\tau+1}-\x_{\tau+1}')\cdot(\x_\tau-\x_\tau')|\leq \frac{\tau}{\tau+1}\|\x_{\tau+1}-\x_{\tau+1}'\|_2\|\x_{\tau}-\x_{\tau}'\|_2.$$
Lemma now follows after simplification and using induction hypothesis. 
\end{itemize}
\end{proof}

==> formulation.tex <==
%%\vspace*{-7pt}
\subsection{Problem Formulation}
%%\vspace*{-7pt}
In this section we formally describe the privacy preserving Online Convex Programming (\ocp) problem. Let $\C\subseteq \mathbb{R}^d$ be a bounded convex set and let $F=\langle f_1, f_2,\dots, f_T\rangle$ be an arbitrary sequence of functions where $f_t:\C\rightarrow \mathbb{R},\ \forall t$. Now, Online Convex programming (\ocp) \cite{Zin} requires an algorithm to select a feasible point $\x_t\in \C$ at the $t$-th step, for which the algorithm incurs a cost of $f_t(\x_t)$, only after which the function $f_t$ is revealed to the algorithm. Then, the algorithm can select next point $\x_{t+1}$ depending on the previous iterates $\langle\x_\tau, 1\leq \tau\leq t\rangle$ and functions $\langle f_\tau, 1\leq \tau \leq t\rangle$. Alternatively, an \ocp algorithm $\A$ maps a function sequence $F$ to a sequence of points $X=\langle\x_1, \x_2, \dots, \x_{T}\rangle \in \C^T$, \ie $\A(F)=X$.

Now, the objective is to minimize the total cost incurred with respect to (w.r.t.) the optimal point $\x^*\in \C$ in hind-sight, i.e., minimize the {\bf regret} defined as: $$\R(T)=\sum_{t=1}^Tf_t(\x_t)-\min_{\x\in \C} \sum_{t=1}^Tf_t(\x).$$

Typically, the goal is to get a sub-linear regret bound, i.e., $\lim_{T\rightarrow\infty}\frac{1}{T}\R(T)=0$ as this implies that the online solution is no worse than the optimal offline solution in the limit as $T \rightarrow \infty$.

Now, we specify the model and the notion of differentially privacy that we use to guarantee privacy of our algorithms. Let each function $f_t$ be held by a party that does not want to reveal information about it.
%wants to remain anonymous.
Furthermore, we assume that the computation of the algorithm is inaccessible to an external observer. However, the output of the algorithm {\em after each step} is visible externally. Thus, to make our method differentially private over the complete sequence of functions, we need to ensure that the output of the algorithm at {\em each step} $t$ preserves differential privacy of the function sequence $f_1, \dots, f_t$. %Intuitively, this means that changing an $f_\tau, \tau\leq t$ to some other function $f'_\tau$ will not modify $\x_{t+1}$ by a large amount. That is, individual cost functions are indistinguishable to an an external observer. %If the output of the algorithm remains more or less the same, any external observer cannot infer anything about about the cost functions input to the algorithm. We provide below the formal definition of differential privacy of an algorithm below.
We now formally define the notion of differential privacy in the context of our problem.
\begin{defn}[$(\epsilon,\delta)$-differential privacy~\cite{DMNS,ODO}]
\label{def:dp}
A randomized \ocp\ algorithm $\mathcal{A}$ is $(\epsilon,\delta)$-differentially private if given any two function sequences $F$ and $F'$ (of size $T$) differing in {\bf exactly} one cost function, for all $\mathcal{S}\subset \C^{T}$ the following holds:
$$\Pr[\mathcal{A}(F)\in \mathcal{S}]\leq e^\epsilon\Pr[\mathcal{A}(F')\in \mathcal{S}]+\delta$$
\end{defn}
%<<<<<<< .mine
Intuitively, the above definition means that changing an $f_\tau, \tau\leq t$ to some other function $f'_\tau$ will not modify the output at each step $\x_{t+1}$ by a large amount.\\ %an algorithm is differentially private if small change in its input do not lead to significant changes in the output. For the \ocp\ problem we need to output an iterate $\x_t$ at each step, so each step needs to be differentially private w.r.t. change in any $f_\tau, 1\leq \tau\leq t$, {\em however} overall there can be only one total change in the function sequence $F$. \\
{\bf Notations}\\
%We use bold-face small letters for vectors and  block letters for matrices. We denote the subsequence of $F$ till the $t$-th step as $F_t=\langle f_1, \dots, f_t\rangle$. $d$ is the dimensionality of ambient space of $\C$. $\alpha$ is  the minimum strong convexity parameter of any $f_t\in F$. $L$ is the largest Lipschitz constant of any $f_t \in F$ and  $L_G$  the largest Lipschitz constant of the gradient of any $f_t\in F$ (if exists). The non-private and private versions of an \ocp algorithm output $\x_{t+1}$ and $\hat{\x}_{t+1}$ respectively, at time step $t$. $\x^*$ denotes the optimal offline solution, that is $\x^* = \argmin_{\x in \C} \sum_{t = 1}^T f_t(\x)$.  $\R_{\A}$ denotes the regret of an OCP  algorithm $\A$.
We use bold-face small letters for vectors and  block letters for matrices. We denote the subsequence of $F$ till the $t$-th step as $F_t=\langle f_1, \dots, f_t\rangle$. $d$ is the dimensionality of ambient space of $\C$. $\alpha$ is  the minimum strong convexity parameter of any $f_t\in F$. Similarly, $L$ and $L_G$ are the largest Lipschitz constant and the Lipschitz constant of gradient of any $f_t\in F$. Recall that a function $f:\C\rightarrow\mathbb{R}$ is $\alpha$-strongly convex, if for all $\gamma\in (0,1)$ and for all $\x,\bm y\in\C$ the following holds: $f(\gamma\x+(1-\gamma)\bm y)\leq \gamma f(\x)+(1-\gamma) f(\bm y)-\frac{\alpha}{2}\ltwo{\x-\bm y}^2$. Also recall that a function $f$ is $L$-Lipschitz, if for all $\x,\bm y\in\C$ the following holds: $|f(\x)-f(\bm y)|\leq L\ltwo{\x-\bm y}$. Non-private and private versions of an \ocp algorithms output $\x_{t+1}$ and $\hat{\x}_{t+1}$ respectively, at time step $t$. $\x^*$ denotes the optimal offline solution, that is $\x^* = \argmin_{\x \in \C} \sum_{t = 1}^T f_t(\x)$.  $\R_{\A}$ denotes the regret of an OCP  algorithm $\A$.

%Intuitively, an algorithm is differentially private if small change in its input do not lead to significant changes in the output. For the \ocp\ problem we need to output an iterate $\x_t$ at each step, so each step needs to be differentially private w.r.t. change in any $f_\tau, 1\leq \tau\leq t$, {\em however} overall there can be only one total change in the function sequence $F$. \\
%{\bf Notation}\\
%We fix some  notation which we use throughout the paper. We use bold-face small letters for vectors and  block letters for matrices, for example $\x$ is a vector and $V$ is a matrix. We do interchangibly use block letters to represent vectors or sets whenever the context is clear.
%
%Let $\C$( usually in $ \mathbb{R}^d$) where $d$ is the dimensionality,  represent a bounded convex set in which the set of output vectors of the {\it Online Convex Programming} (\ocp) algorithm lie. $F=\{f_1, f_2,\dots, f_T\}$ be a sequence of functions where $f_t:\C\rightarrow \mathbb{R}, \forall t$ represents a sequence of functions (costs) indexed by the time $t$. $\alpha$ is the minimum strong convexity of the cost functions $f_t$ involved. For the output of the \ocp algorithms at time $t$ we use the notation $x_t$ and $\hat{x}_t$. These refer to the outputs of the non-private and the private versions of the algorithm in the context respectively. $d$ is the dimensionality of the range of the cost functions(data). $\R_{\A}$ is the regret of an OCP  algorithm $\A$.

%\section{Notation}
%We fix some  notation which we use throughout the paper. We use bold-face small letters for vectors and  block letters for matrices, for example $\x$ is a vector and $V$ is a matrix. We do interchangibly use block letters to represent vectors or sets whenever the context is clear.

%Let $\C$( usually in $ \mathbb{R}^d$) where $d$ is the dimensionality,  represent a bounded convex set in which the set of output vectors of the {\it Online Convex Programming} (\ocp) algorithm lie. $F=\{f_1, f_2,\dots, f_T\}$ be a sequence of functions where $f_t:\C\rightarrow \mathbb{R}, \forall t$ represents a sequence of functions (costs) indexed by the time $t$. $\alpha$ is the minimum strong convexity of the cost functions $f_t$ involved. For the output of the \ocp algorithms at time $t$ we use the notation $x_t$ and $\hat{x}_t$. These refer to the outputs of the non-private and the private versions of the algorithm in the context respectively. $d$ is the dimensionality of the range of the cost functions(data). $\R_{\A}$ is the regret of an OCP  algorithm $\A$.
%>>>>>>> .r104
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "nips2011"
%%% End:


==> ftl.tex <==
\section{Follow the Leader}
\label{sec:FTL}
As another application of Algorithm \ref{alg:ocp_diff} we describe our Private Follow The Leader Algorithm (\pftl). It is based on the Follow The Leader algorithm (\ftl\,) by \cite{HKKA}. \ftl\, at each time step $t+1$ outputs $\x_{t+1}=\argmin_{\x\in\C}\frac{1}{t}\sum_{\tau=1}^t f_{\tau}(\x)$. The first vector $\x_1\in\C$ is chosen  arbitrarily without querying the data set.  For \pftl\ we instantiate the non-private algorithm $\A$ (in Algorithm \ref{alg:ocp_diff}) with the following. Let $\mathcal{A}(F_t)=\argmin_{\x\in\C}\frac{1}{t}\sum_{\tau =1}^t f_{\tau}(\x)$, where $F_t=\langle f_1,\cdots,f_t\rangle$. We assume the following regarding the cost functions.
\begin{enumerate}
	\item The cost function $f_t(\x)$ can be written as $g_t(\langle \bm v_t,\x\rangle)+\frac{\alpha}{2}\ltwo{\x}^2$, where $g_t:\mathbb{R}\rightarrow\mathbb{R}$ is a univariate function and $\bm v_t$ is a vector s.t. $\ltwo{\bm v_t}\leq R$ (a constant). We need this condition for our regret bound.
	\item The cost function $f_t(\x)$ is $L$-Lipschitz in $\x$,~\emph{i.e.,} $|f_t(\x_1)-f_t(\x_2)|\leq L\ltwo{\x_1-\x_2},\forall \x_1,\x_2\in \C$.
	\item A relatively mild assumption is that the \emph{origin} ($\0^d$) is contained in the convex set $\C$.
\end{enumerate}

Our first lemma is about bounding the sensitivity of $\mathcal{A}(F_t)$.

\begin{lemma}
$L_2$-sensitivity of $\x_{t+1}=\argmin_{\x\in\C}\frac{1}{t}\sum_{\tau =1}^t f_{\tau}(\x)$ is $\frac{2L}{t\alpha}$.
\end{lemma}

\begin{proof}
$\x_{t+1}=\arg\min_{\x\in\C}\frac{1}{t}\sum_{\tau =1}^t f_{\tau}(\x)$ is the result of a constrained convex optimization on the convex set $\C$. For the ease of representation let $G_{t}(\x)=\frac{1}{t}\sum_{\tau=1}^t f_{\tau}(\x)$ . Let $G_t'$ be another summation where $G_t$ and $G_t'$  differ in exactly one of it summands. Let $\x'_{t+1}\in\C$ be the vector that minimizes $G'_{t}$.

For all points $y\in\C$, the following are true,
\begin{enumerate}
	\item $\subg{G_{t}}(\x_{t+1})^T(y-\x_{t+1})\geq 0$
	\item $\subg{G'_{t}}(\x'_{t+1})^T(y-\x'_{t+1})\geq 0$
\end{enumerate}
where $\subg{}$ is any subgradient of the function $G_t$ or $G_{t'}$.
The cost functions  $f_t$ are assumed to be $\alpha$-strongly convex. Thus, both $G_{t}$ and $G'_{t}$ are $\alpha$-strongly convex.
Thus, we have
\begin{eqnarray*}
&&G_t(\x'_{t+1})\geq G_t(\x_{t+1})+\frac{\alpha}{2}\ltwo{\x'_{t+1}-\x_{t+1}}^2\\
&&G'_t(\x_{t+1})\geq G'_t(\x'_{t+1})+\frac{\alpha}{2}\ltwo{\x'_{t+1}-\x_{i+1}}^2\\
\end{eqnarray*}
Combining the above two equations we have,
$$\alpha\ltwo{\x'_{t+1}-\x_{t+1}}^2\leq (G_t(\x'_{t+1})-G'_t(\x'_{t+1}))+(G'_t(\x_{t+1})-G_t(\x_{t+1}))$$
Let the summands of $G_t$ and $G'_k$ differ at position $k$. Therefore, $G_t(\x'_{t+1})-G'_t(\x'_{t+1})=\frac{1}{t}(f_k(\x'_{t+1})-f'_k(\x'_{t+1}))$ and $G'_t(\x_{t+1})-G_t(\x_{t+1})=\frac{1}{t}(f'_k(\x_{t+1})-f'_k(\x_{t+1}))$.
where $f'_k$ is another function differing from $f_k$.
Hence,
\begin{eqnarray}
&&\alpha\ltwo{\x'_{t+1}-\x_{t+1}}^2\leq\frac{1}{t}\left(f_k(\x'_{t+1})-f'_k(\x'_{t+1})+f'_k(\x_{t+1})-f_k(\x_{t+1})\right)\\
&&\leq \frac{2L}{t}\ltwo{\x'_{t+1}-\x_{t+1}}
\end{eqnarray}
The last inequality follows from the Lipschitz property of the cost function $f_t$.
Finally,
$$\ltwo{\x'_{t+1}-\x_{t+1}}\leq \frac{2L}{t\alpha}$$
\end{proof}

We fix $\lambda_\mathcal{A}=\frac{2L}{\alpha}$ in Algorithm~\ref{alg:ocp_diff} as the sensitivity parameter.

\begin{corollary}[Privacy]
Private \ftl\, is $(3\epsilon,2\delta)$-differentially private.
\end{corollary}
The proof of this corollary follows directly from Theorem \ref{Thm:GenPri}.

Before we state the regret bound for \pftl, we state the following theorem bounding the regret for non-private \ftl\, (\ie when we do not add noise to the output).  The proof can be obtained (with minor modification) from the regret bound analysis of the version of \ftl\, by  \cite{HAS}.

\begin{thm}[Regret bound for \ftl\,]
Assume that for all $t$, the function $f_t(x)$ can be written as $g_t(\langle v_t,\x\rangle)+\frac{\alpha}{2}\ltwo{\x}^2$ for a univariate convex function $g_t(\langle v_t,\x\rangle)$ and some vector $v_t\in\mathbb{R}^p$. Assume that for some $R,G >0$, we have $\ltwo{v_t}\leq R$ and for all $\x\in\C$, we have $| g'_t(\langle v_t,\x\rangle)|\leq G$ and $|g''_t(\langle v_t,\x\rangle)|\geq 0$. Also assume that the convex set $\C$ contains the origin. The  non-private \ftl\, over $T$ rounds has~\emph{regret}
$$\leq \frac{1}{\alpha}\left(G\ R+C\alpha\right)^2\ln T$$
where $C$ is the diameter of the convex set $\C$.
\label{Thm:UtilKalai}
\end{thm}

We now state the regret bound for \pftl. It follows as a corollary from Theorem~\ref{thm:util}.

\begin{corollary}[Regret bound for \pftl\,]
Suppose for all $t$, $f_t$ satisfies all the conditions in theorem  \ref{Thm:UtilKalai} Let the Lipschitz constant of $f_t$ for all $t$ be at most $L$. Then, the expected regret (\emph{i.e.,} $\E[\sum_{t=1}^Tf_t(\hat\x_t)]-\min_{\x\in\C}\sum_{t=1}^T f_t(\x))$  is upper bounded by
$$\frac{1}{\alpha}\left(\left(G R+C\alpha\right)^2\ln T+4\sqrt{d} L^2\sqrt{T}\frac{\ln^2\frac{2}{\delta}}{\sqrt \epsilon}\right)$$
where $C$ is the diameter of the convex set $\C$ and $d$ is the dimensionality of the output space.
\end{corollary} 

==> general.tex <==

\subsection{Privacy Guarantee for Private Online Convex Programming}
\label{Sec:OCP1}
\label{sec:OCPPriv}
Note that every step of our private algorithm adds noise proportional to the sensitivity of the algorithm at that step to obfuscate the output, so as to provide privacy guarantee for that particular step. We make the claim precise in the following lemma. 
\begin{lemma}
Let $c>0$ be any constant, and $\beta=\lambda_\A T^{0.5+c}\sqrt{\frac{2}{\epsilon}\left(\ln\frac{T}{\delta}+\frac{\sqrt{\epsilon}}{T^{0.5+c}}\right)}$. Then step $t$ of algorithm~\ref{alg:ocp_diff}, i.e., $t$-th step output $\hatx_{t+1}$ is $(\frac{\sqrt\epsilon}{T^{0.5+c}},\frac{\delta}{T})$-differentially private.
\label{Lem:SingGenPriv}
\end{lemma}

\begin{proof}
As the output $\hatx_{t+1}$ is just a projection, i.e., a function (independent of the input functions $F$) of $\tx_{t+1}$, hence $(\epsilon, \delta)$-differential privacy for $\tx_{t+1}$ would imply the same for $\hatx_{t+1}$.
 
Now by the definition of differential privacy (see Definition~\ref{def:dp}), $\txt$ is $(\epsilon_1, \frac{\delta}{T})$-differential private, if for any measurable set $\Omega\subseteq\mathbb{R}^{p}$:
$$\Pr[\txt\in \Omega]\leq e^{\epsilon_1}\Pr[\txt'\in \Omega]+\delta/T,$$
where $\txt=\xt+b$ is the output of the noise additions step (see Algorithm~\ref{alg:ocp_diff}, Step 7) of our differentially private algorithm $\A_P$, when applied to function sequence $F_t=\langle f_1, \dots, f_t\rangle$. Similarly, $\txt'=\xt'+b$ is the output of the noise addition to $\xt'$ which is obtained by applying update step to $F_t'$ where $F_t'$ differs from $F_t$ in exactly one function entry. 

Now, $\txt\sim {\mathcal N}(\x_{t+1},\frac{\beta^2}{t^2} \mathbb{I}^d)$ and $\txt'\sim {\mathcal N}(\x_{t+1}', \frac{\beta^2}{t^2} \mathbb{I}^d)$. Hence:
\begin{eqnarray*}
\frac{\Pr[\txt\in \Omega]}{\Pr[\txt'\in \Omega]}=\frac{\int_{\x\in \Omega}\pdf(\txt=\x)}{\int_{\x\in \Omega}\pdf(\txt'=\x)}=\frac{\int_{\x\in \Omega}\exp\left(-\frac{\ltwo{\x-\xt}^2}{2\frac{\beta^2}{t^2}}\right)d\x}{\int_{\x\in \Omega}\exp\left(-\frac{\ltwo{\x-\xt'}^2}{2\frac{\beta^2}{t^2}}\right)d\x}
\end{eqnarray*}
%Let $b=\theta-\mathcal{M}_i(T_i)$, and $f=\mathcal{M}_i(T'_i)-\mathcal{M}_i(T_i)$. We have


Let $\dxt=\xt-\xt'$. Next, we bound each individual term in the above integration: 
\begin{align}
  \frac{\exp\left(-\frac{t^2 \ltwo{\x-\xt}^2}{2\beta^2}\right)}{\exp\left(-\frac{t^2\ltwo{\x-\xt'}^2}{2\beta^2}\right)}&=\exp\left(\frac{t^2}{2\beta^2}\dxt^T(2\x-\xt-\xt')\right),\nonumber\\
&=\exp\left(\frac{t^2}{2 \beta^2}\left(2\dxt^T(\x-\xt)-\|\dxt\|_2^2\right)\right), \nonumber\\
&\leq \exp\left(\frac{t^2}{2 \beta^2 }\left(2|\dxt^T(\x-\xt)|+\|\dxt\|_2^2\right)\right), \nonumber\\
&\leq \exp\left(\frac{t^2}{\beta^2}|\dxt^T(\x-\xt)|\right)\exp\left(\frac{\lambda_\A^2}{2\beta^2}\right), 
\label{eq:HPB}
\end{align}
where the last inequality follows from the sensitivity assumption~\eqref{eq:sens_ocp}. 

Since $\txt\sim\mathcal{N}(\xt,\frac{\beta^2}{t^2}\I_p)$, we have $(\txt-\xt)^T\dxt\sim\mathcal{N}(0,\frac{\beta^2}{t^2}\|\dxt\|_2^2)$. %Using the maximum value of $f$ (from the assumption on the sensitivity of $\mathcal{A}(T_i))$, we analyze the worst case,~\emph{i.e.,} we assume $\langle b,f\rangle\sim\mathcal{N}(0,\frac{\beta^2\lambda^2}{i^2})$. 
Now, using \eqref{eq:sens_ocp} and Mill's inequality, $$\Pr[|(\txt-\xt)^T\dxt|\geq \frac{\beta\lambda_\A}{t^2}z]\leq \Pr[|(\txt-\xt)^T(\dxt)|\geq\frac{\beta}{t}\|\xt-\xt'\|z]\leq e^{-\frac{z^2}{2}},$$ where $z>0$. Setting R.H.S. $\leq\frac{\delta}{T}$, we have $z\geq\sqrt{2\ln\frac{T}{\delta}}$. 

We call the set of $\txt\in \Omega$ to be the ``good set'' $\G$ if 
\begin{equation}
\label{eq:good}
(\txt-\xt)^T\dxt\geq\frac{\beta\lambda_\A}{t^2}z.
\end{equation}
Using the above bound, $\Pr[\txt\not\in \G]\leq \frac{\delta}{T}$ and for all $\x\in \G$:
\begin{align}
\exp\left(\frac{t^2}{\beta^2}|\dxt^T(\x-\xt)|\right)\exp\left(\frac{\lambda_\A^2}{2\beta^2}\right)&\leq \exp\left(\frac{\lambda_\A^2}{2\beta^2}+\frac{\lambda_\A}{\beta}\sqrt{2\ln\frac{T}{\delta}}\right),\nonumber\\
&\leq e^{\epsilon_1},
\label{eq:expupg}
\end{align}
where $\epsilon_1=\frac{\sqrt\epsilon}{T^{0.5+c}}$ and $\beta$ is as given in the Lemma statement. 

Similarly, we can define set $\G'$ for $\txt'$ and furthermore, 
\begin{equation}
  \label{eq:gg}
  \Pr[\txt\in\G]=\Pr[\txt'\in \G'].
\end{equation}
Combining \eqref{eq:HPB} and \eqref{eq:expupg}:
\begin{equation}
  \label{eq:ogog}
  \Pr[\txt\in\Omega|\txt\in \G]\leq e^{\epsilon_1}\Pr[\txt'\in \Omega|\txt'\in \G'].
\end{equation}
Using \eqref{eq:gg} and \eqref{eq:ogog}:
\begin{align}
  \Pr[\txt\in \Omega]&\leq \Pr[\txt\in \Omega|\txt\in \G]\Pr[\txt\in \G]+\Pr[\txt\not\in \G],\nonumber\\
& \leq e^{\epsilon_1} \Pr[\txt'\in \Omega|\txt\in \G]\Pr[\txt'\in \G]+\delta, \nonumber\\
& \leq e^{\epsilon_1} \Pr[\txt'\in \Omega]+\delta. 
\label{eq:txtx}
\end{align}
Hence, proved. 
\end{proof}

The above lemma shows $(\frac{\sqrt\epsilon}{T^{0.5+c}},\frac{\delta}{T})$-differential privacy for each step of the \ocp\ algorithm. To prove the privacy of our online Algorithm \ref{alg:ocp_diff} over {\em all} $T$-iterations we use the following lemma by \cite{DRV}. Our proof strategy from here on is inspired from a proof technique developed by \cite{HR}. 

\begin{lemma}[\cite{DRV}]
Suppose two random variables $Y$ and $Z$ satisfy $$D_\infty(Y||Z)=\max_{w\in\supp(Y)}\ln\left(\frac{\pdf[Y=w]}{\pdf[Z=w]}\right)\leq\epsilon,\ \ \ D_{\infty}(Z||Y)\leq\epsilon.$$ Then $D(Y||Z)=\int_{w\in\supp(Y)}\pdf[Y=w]\ln\left(\frac{\pdf[Y=w]}{\pdf[Z=w]}\right)\leq 2\epsilon^2$. Here $supp(Y)$ is the support set of a random variable $Y$.
\label{lem:Dwork}
\end{lemma}

We now state a technical lemma which will be useful for our privacy. 

\begin{lemma}
Assuming that at each stage $T$,  algorithm~\ref{alg:ocp_diff} preserves $\frac{\sqrt{\epsilon}}{T^{0.5+c}}$-differential privacy, $$\E_{ \txt}\left[\ln\left(\frac{\pdf[\txt]}{\pdf[\txt'=\txt]}\right)\right]\leq\frac{2\epsilon}{T^{1+2c}},$$
where $\txt$ and $\txt'$ are output of the $t$-th time step Noise Addition Step of our private ocp\ algorithm (Algorithm~\ref{alg:ocp_diff}), when applied to function sequences $F_t$ and $F_t'$ differing in exactly one function entry. 
\label{lem:pro}
\end{lemma}
\begin{proof}
Using the fact that $\txt$ is $\frac{\sqrt{\epsilon}}{T^{0.5+c}}$-differential private: 
$$\forall \x,\hspace{0.1cm}-\frac{\sqrt{\epsilon}}{T^{0.5+c}}\leq\ln\left(\frac{\pdf[\txt=\x]}{\pdf[\txt'=\x]}\right)\leq \frac{\sqrt{\epsilon}}{T^{0.5+c}}.$$
Lemma now follows using the above observation with Lemma~\ref{lem:Dwork}. 
\end{proof}
 
Finally, we state the privacy guarantee for algorithm~\ref{alg:ocp_diff} over all the $T$-iterations.
\begin{thm}[Privacy \ocp]
The Private \ocp\ algorithm (see Algorithm~\ref{alg:ocp_diff}) is $(3\epsilon,2\delta)$-differentially private.
\label{Thm:GenPri}
\end{thm}

\begin{proof}
Following the notation from the proof of lemma~\ref{Lem:SingGenPriv} we define the ``good'' set $\G$ (see \eqref{eq:good}). Now, using \eqref{eq:gg} and Lemma~\ref{Lem:SingGenPriv}, for each round, 
\begin{equation}
\Pr[\txt\in\G]=\Pr[\txt'\in \G']=\frac{\delta}{T}.   
\end{equation}
Now, probability that the noise vector $\b=\txt-\xt=\txt'-\xt'$ always leads to ``good'' set in all $T$ rounds is $T\cdot \frac{\delta}{T}=\delta$. 

Now, we condition the remaining proof on the fact that the noise vector $\b$ in each round is such that $\tx_t\in \G$ and $\tx_t'\in \G'$. 

Let $L(\tx_1,\cdots,\tx_T)=\sum_{t=1}^T\ln\left(\frac{\pdf(\tx_t)}{\pdf(\tx_t'=\tx_t)}\right)$, where each $\x_t\in\mathbb{R}^d$.

Therefore, by Lemma~\ref{lem:pro}, $$\E[L(\tx_1,\cdots,\tx_T)]=\sum_{t=1}^T \E_{\tx_t}\left[\ln\left(\frac{\pdf(\tx_t)}{\pdf(\tx_t'=\tx_t)}\right)\right]\leq \frac{2T\epsilon}{T^{1+2c}}\leq\frac{2\epsilon}{T^{2c}}\leq 2\epsilon.$$

Let $Z_t=\ln\left(\frac{\pdf(\tilde{x}_t=\xt)}{\pdf(\tilde{x}_t'=\x_t)}\right)$. Since the randomness is freshly added in each iteration, $Z_t$ are independent. We have $L(\x_1,\cdots,\x_T)=\sum_{t=1}^T Z_t$, where $|Z_t|\leq\frac{\sqrt{\epsilon}}{T^{0.5+c}}$. By Azuma-Hoeffding's inequality
\begin{align*}
\Pr[L(\tx_1,\cdot,\tx_T)\geq 2\epsilon+\epsilon]&\leq 2\exp\left(\frac{-2\epsilon^2}{T\times\frac{\epsilon}{T^{1+2c}}}\right),\\
&\leq 2\exp\left(-2T^{2c}\right).
\end{align*}
Let $\delta=2\exp\left(-2T^{2c}\right)$. We have $-2T^{2c}=\ln\frac{\delta}{2}$. Solving for $c$ we get $c=\frac{(\ln (\frac{1}{2}\ln \frac{2}{\delta} )}{2\ln T}$.

Hence, with probability $1-\delta$, $3\epsilon$-differential privacy holds conditioned on $\tx_t\in\G$ and $\tx_t'\in\G'$, i.e, 
$$\forall\x, \hspace{0.1cm}\Pi_{t=1}^T\pdf(\x_t=\x)\leq e^{3\epsilon}\Pi_{t=1}^T\pdf(\tx_t'=\x).$$
Also, recall that with probability $1-\delta$, our noise vector $\b$ in each round itself was such that $\tx_t\in \G$ and $\tx_t'\in \G'$. Theorem now follows using an argument similar to \eqref{eq:txtx}. 
\end{proof}


\subsection{Generic Regret Bound Analysis for OCP}
\label{sec:OCPReg}
In this section, we provide a generic regret bound analysis for Algorithm \ref{alg:ocp_diff}. The regret of our private \ocp\ algorithm depends on the regret $\R_\A(T)$ the non-private learning algorithm $\A$.

\begin{thm}[Regret Bound]
Let $L>0$ be the maximum Lipschitz constant of any function $f_t$ in the sequence $F$, %and let $\alpha>0$ be the minimum strong convexity parameter of any function $f_t$ in $F$. 
 and let the regret of the non-private \ocp\ algorithm $\A$ over $T$-time steps is $\R_{\A}(T)$ and let $\lambda_\A$ be the sensitivity parameter of $\A$ (see \eqref{eq:sens_ocp}), then the expected regret of our Private \ocp\ algorithm (Algorithm~\ref{alg:ocp_diff}) follows:
$$\E\left[\sum_{t=1}^Tf_t(\hat\x_t)\right]-\min_{\x\in\C}\sum_{t=1}^Tf_t(\x)\leq 2dL\lambda_\A\sqrt{T}\frac{\ln^2\frac{T}{\delta}}{\sqrt{\epsilon}}+\R_{\A}(T),$$  
%is upper bounded by 
%$$\R_{\A}(T)+\lambda_\A \sqrt{T\ln\sqrt{\frac{2}{\delta}}}\sqrt{\frac{2}{\epsilon}\left(\ln\frac{T}{\delta}+\frac{\sqrt{\epsilon}}{\sqrt{T\ln\sqrt{\frac{2}{\delta}}}}\right)}\left(\frac{\sqrt{2}\Gamma((d+1)/2)\ln T}{\Gamma(d/2)}\right),$$
where $d$ is the dimensionality of the output space. That is, the regret bound is $ R_\A(T)+\tilde{O}\left(d\sqrt{T}\right)$. 
\label{thm:util}
\end{thm}  

\begin{proof}
Let $\hat\x_1,\cdots,\hat  \x_T$ be the output of the POCP algorithm~\ref{alg:ocp_diff}. By the Lipschitz continuity of the cost functions $f_t$ we have
\begin{eqnarray}
&&\sum_{t = 1}^T f_t(\hat{\x}_t)-\min_{\x\in\C}\sum_{t=1}^Tf_t(\x) \leq \sum_{t = 1}^T f_t(\x_t)-\min_{\x\in\C}\sum_{t=1}^Tf_t(\x) + L \sum_{t = 1 }^T \ltwo{\hat{\x}_t - \x_t}\\
&&= R_\A(T) +  L \sum_{t = 1 }^T \ltwo{\hat{\x}_t - \x_t}.
\label{eq:rahx}
\end{eqnarray}
Since at any time $t$,  $\hat\x_{t}$ is the projection of $\tilde\x_{t}$ on the convex set $\C$, we have $$\ltwo{\x_t-\hat\x_t}\leq\ltwo{\x_t-\tilde{\x}_t}=\ltwo{\b_t},$$ where $\b_t$ is the noise vector added at in the $t^{th}$ iteration of algorithm~\ref{alg:ocp_diff}. Therefore,
\begin{equation} 
\sum_{t=1}^T L \ltwo{\x_{t}-\hat\x_{t}}\leq L \sum_{t =1}^T\ltwo{\b_{t}}.
\label{eq:hxb}
\end{equation}
Now, $\b_{t} \sim \mathcal{N} ( \0^d, \frac{\beta^2}{t^2} \I^d) $ where $$\beta= \lambda_{\A}T^{0.5+c}\sqrt{\frac{2}{\epsilon}\left(\ln\frac{T}{\delta}+\frac{\sqrt{\epsilon}}{T^{0.5+c}}\right)}.$$
 
Therefore, $\ltwo{\b_{t}}$ follows Chi-distribution with parameters $\mu=\frac{\sqrt{2}\frac{\beta}{t} \Gamma((d+1)/2)}{\Gamma(d/2)}$ and $\sigma^2=\frac{\beta^2}{t^2}(d-\mu^2)$. 

Using $c = \frac{\ln{ (\frac{1}{2}\ln{\frac{2}{\delta}})} }{2\ln{T}}$,
\begin{align}
 \E[\sum_{\tau=1}^T\ltwo{\b_{\tau}}] &\leq \frac{\sqrt{2}\beta \Gamma((d+1)/2)}{\Gamma(d/2)} \int_{\tau =1}^T \frac{1}{t}d\tau, \nonumber\\
&= \frac{\Gamma((d+1)/2)}{\Gamma(d/2)} \lambda_\A\sqrt{T}\ln {T}\sqrt{\frac{2}{\epsilon}\ln{\frac{2}{\delta}}\left(\ln\frac{T}{\delta}+\frac{\sqrt{\epsilon}}{\sqrt{\frac{T}{2}\ln{\frac{2}{\delta}}}}\right)},\nonumber\\
&\leq 2d\lambda_\A\sqrt{T}\frac{\ln^2\frac{T}{\delta}}{\sqrt{\epsilon}}. 
\label{eq:noisenorm}
\end{align}
The theorem now follows by combining \eqref{eq:rahx}, \eqref{eq:hxb}, \eqref{eq:noisenorm}. 
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "nips2011"
%%% End: 


==> lin.tex <==
%\subsection{Linearization Method}
%%%\vspace*{-7pt}
\subsection{Implicit Gradient Descent Algorithm}
%%%\vspace*{-7pt}
\label{sec:IGD}
We first describe the \igd\ algorithm and then show how it can be modified to preserve differential privacy. \igd\ \cite{KB10} maintains just the current iterate $\x_t$ and given a new function $f_t$, finds the new iterate $\x_{t+1}$ so that it not ``far'' away from the current iterate but at the same time tries to minimize the cost $f_t(\x_{t+1})$. Formally,
\begin{equation*}
  \x_{t+1}\leftarrow \argmin_{\x\in \C} \left(D_\phi(\x,\x_t)+\eta_t f_t(\x)\right),
\end{equation*}
where $D_\phi(\cdot,\cdot)$ is the Bregman divergence generated by function $\phi$. Now, selecting $D_\phi(\cdot,\cdot)$ to be the squared Euclidean distance implies the following:
\begin{equation}
  \x_{t+1}\leftarrow \argmin_{\x\in \C} \frac{1}{2}\ltwo{\x-\x_t}^2+\eta_t f_t(\x),
  \label{eqn:abc1}
\end{equation}
We assume each $f_t(x)$ is $\alpha$-strongly convex and $L$-Lipschitz w.r.t. $\x$. Under these assumptions, \cite{KB10} show $O(\log T)$ regret for \igd. 

Now, recall that, a differentially private algorithm should be stable, \ie changing one single function in the sequence $F$ should not effect the output sequence significantly. Hence, to show differential privacy for \igd, we first needs to show that it is not very ``sensitive'' to previous cost functions. To this end, we first formalize the notion of sensitivity of an \ocp\ algorithm. 
\begin{defn}[$L_2$-sensitivity~\cite{DMNS,CM}]
Let $F,F'$ be two function sequences differing in at most one entry, i.e., at most one function can be different. Then, the sensitivity of an algorithm~$\mathcal{A}:F\rightarrow\C^T$ is the difference in the $T$-th output $\x_T=\A(F)_T$ of the algorithm $\A$, i.e, 
$${\mathcal S}(\mathcal{A})=\sup_{F,F'}\ltwo{\mathcal{A}(F)_T-\mathcal{A}(F')_T}$$
%%%%\vspace*{-20pt}
\label{defn:sensitivity}
\end{defn}
Having defined the notion of sensitivity formally, we now bound sensitivity of \igd\ at each step. 
\begin{lemma}[{\bf \igd\ Sensitivity}]
\label{lemma:sens_igd}
Sensitivity of the \igd\ algorithm is $\frac{2L}{t}$ for the $t$-th iterate, where $L$ is the maximum Lipschitz constant of any function $f_{\tau}, 1\leq \tau\leq t$. 
%%%\vspace*{-3pt}
\end{lemma}
\begin{proof}
We prove the above lemma using mathematical induction. \\
{\bf Base Case ($t=1$)}: As $\x_1$ is selected randomly, it's value doesn't depend on the underlying dataset. \\
{\bf Induction Step $t=\tau+1$}: As $f_\tau$ is $\alpha$ strongly convex. The total convexity of the function $$\tilde{f}_\tau(\x)=\frac{1}{2}\|\x-\x_{\tau}\|_2^2+\eta_\tau f_\tau(\x),$$ 
is $\frac{\tau+1}{\tau}$. Now using strong convexity and the fact that at optima $\x_{\tau+1}$,
$$\partial \tilde{f}_\tau(\x_{\tau+1}) (\x-\x_{\tau+1})\geq 0, \forall \x\in \C,$$
we get:
\begin{equation}
  \label{eq:sens_opt_r}
  \tilde{f}_\tau(\x_{\tau+1}')\geq \tilde{f}_\tau(\x_{\tau+1})+\frac{\tau+1}{2\tau}\|\x_{\tau+1}-\x_{\tau+1}'\|_2^2.
\end{equation}
Now, we consider two cases:
\begin{itemize}
\item {\bf $F-F'=\{f_\tau\}$}: Define $\tilde{f}_\tau'(\x)=\frac{1}{2}\|\x-\x_{\tau}\|^2+\eta_\tau f_\tau'(\x)$ and let $\x_{\tau+1}'=\argmin_{\x\in \C} \tilde{f}_\tau'(\x)$. Then, similar to \eqref{eq:sens_opt_r}, we get:
\begin{equation}
  \label{eq:sens_opt_rp1}
  \tilde{f}_\tau'(\x_{\tau+1})\geq \tilde{f}_\tau'(\x_{\tau+1}')+\frac{\tau+1}{2\tau}\|\x_{\tau+1}-\x_{\tau+1}'\|_2^2.
\end{equation}
Adding \eqref{eq:sens_opt_r} and \eqref{eq:sens_opt_rp1}, we get:
$$\|\x_{\tau+1}-\x_{\tau+1}'\|_2^2\leq \frac{1}{\tau+1}|f_\tau(\x_{\tau+1}')+f_\tau'(\x_{\tau+1})-f_\tau(\x_{\tau+1})-f_\tau'(\x_{\tau+1}')|\leq \frac{2L}{\tau+1}\|\x_{\tau+1}-\x_{\tau+1}'\|_2.$$
Lemma now follows using simplification. 
\item {\bf $F-F'=\{f_i\},\ i<\tau$}: Define $\tilde{f}_\tau'(\x)=\frac{1}{2}\|\x-\x_\tau'\|^2+\eta_\tau f_\tau(\x)$ and let $\x_{\tau+1}'=\argmin_{\x\in \C} \tilde{f}_\tau'(\x)$. Then, similar to \eqref{eq:sens_opt_r}, we get:
\begin{equation}
  \label{eq:sens_opt_rp11}
  \tilde{f}_\tau'(\x_{\tau+1})\geq \tilde{f}_\tau'(\x_{\tau+1}')+\frac{\tau+1}{2\tau}\|\x_{\tau+1}-\x_{\tau+1}'\|_2^2.
\end{equation}
Adding \eqref{eq:sens_opt_r} and \eqref{eq:sens_opt_rp11}, we get:
$$\|\x_{\tau+1}-\x_{\tau+1}'\|_2^2\leq \frac{\tau}{\tau+1}|(\x_{\tau+1}-\x_{\tau+1}')\cdot(\x_\tau-\x_\tau')|\leq \frac{\tau}{\tau+1}\|\x_{\tau+1}-\x_{\tau+1}'\|_2\|\x_{\tau}-\x_{\tau}'\|_2.$$
Lemma now follows after simplification and using induction hypothesis. 
\end{itemize}
\end{proof}
%Note that the update in Equation \ref{eqn:abc1} is similar to the Gradient Infinitesimal Gradient Ascent (GIGA) algorithm \cite{Zin}, but with a critical difference where GIGA {\em linearizes} $f_t(\x)\approx f_t(\x_{t+1})+\x^T\partial_{\x} f_t(\x_t)$. This approximation simplifies the update without any loss in the regret bound guarantees compared to \igd. %However it is not clear upfront how to make GIGA differentially private without further assumptions over and above the assumptions for \igd. 
%However, linearization leads to higher dependence of GIGA on the previous iterates as the (sub)gradient is evaluated at $\x_t$. This makes GIGA slightly more ``unstable'' than \igd.   %Now, GIGA can be sensitive to the previous iterate . %because any change in the previous iterate can lead to significant changes in the current iterate  
%In contrast, \igd\ algorithm is intuitively more ``stable''; . In fact unless all the convex functions $f_t\in F$ are differentiable w.r.t. $\x$, it is not clear how to make GIGA stable.  However we show that under an additional condition of differentiability, a private variant of GIGA exists with low regret (see Section \ref{sec:GIGA}).
\begin{algorithm}[tb]
	\caption{Private Implicit Gradient Descent Method (PIGD)}
	\begin{algorithmic}[1]
		\STATE {\bfseries Input:} Cost function sequence $F=\langle f_1,\cdots,f_T\rangle$ and the convex set $\C$
                \STATE {\bfseries Parameter:} privacy parameters $(\epsilon, \delta)$
		\STATE Choose $\x_1$ and $\hat\x_1$ randomly from $\C$
		\FOR{$t=1$ to $T-1$} 
                \STATE \textbf{Cost:} $L_t(\hat\x_t)=f_t(\hat\x_t)$
                \STATE \textbf{Learning rate:} $\eta_t=\frac{1}{\alpha t}$
                \STATE \textbf{IGD Update:} $\x_{t+1}\leftarrow \argmin_{\x\in \C} \left(\frac{1}{2} \|\x-\x_t\|_2^2+\eta_t f_t(\x)\right)$
                \STATE \textbf{Noise Addition:} $\hat\x_{t+1}\leftarrow \argmin_{\x\in \C}\left(\|\x-\x_{t+1}-\b\|_2^2\right),\ \ \b\sim\mathcal{N}(\0^d,\frac{\beta^2}{t^2}\I^d )$, where $\beta=2 L T^{0.5+c}\sqrt{\frac{2}{\epsilon}\left(\ln\frac{T}{\delta}+\frac{\sqrt{\epsilon}}{T^{0.5+c}}\right)}$ and $c=\frac{\ln\frac{1}{2}\ln(2/\delta)}{2\ln T}$
                \STATE Output $\hat\x_{t+1}$
		\ENDFOR					
	\end{algorithmic}
	\label{alg:igd}
\end{algorithm} 
%Following the general strategy we now show a bound on the sensitivity of the \igd\ algorithm which we then use to show the privacy guarantees. For the proof see section \ref{sec:IGDSensitive} of Appendix. 
%\begin{proof}
%We prove the above lemma using mathematical induction. \\
%{\bf Base Case ($t=1$)}: As $\x_1$ is selected randomly, it's value doesn't depend on the underlying dataset. \\
%{\bf Induction Step $t=\tau+1$}: As $f_\tau$ is $\alpha$ strongly convex. The total convexity of the function $$\tilde{f}_\tau(\x)=\frac{1}{2}\|\x-\x_{\tau}\|^2+\eta_\tau f_\tau(\x),$$ 
%is $\frac{\tau+1}{\tau}$. Now using strong convexity and the fact that at optima $\x_{\tau+1}$,
%$$\partial \tilde{f}_\tau(\x_{\tau+1}) (\x-\x_{\tau+1})\leq 0, \forall \x\in \C,$$
%we get:
%\begin{equation}
%  \label{eq:sens_opt_r}
%  \tilde{f}_\tau(\x_{\tau+1}')\geq \tilde{f}_\tau(\x_{\tau+1})+\frac{\tau+1}{2\tau}\|\x_{\tau+1}-\x_{\tau+1}'\|^2.
%\end{equation}
%Now, we consider two cases:
%\begin{itemize}
%\item {\bf $F-F'=\{f_\tau\}$}: Define $\tilde{f}_\tau'(\x)=\frac{1}{2}\|\x-\x_{\tau}\|^2+\eta_t f_\tau'(\x)$ and let $\x_{\tau+1}'=\argmin_{\x\in \C} \tilde{f}_\tau'(\x)$. Then, similar to \eqref{eq:sens_opt_r}, we get:
%\begin{equation}
%  \label{eq:sens_opt_rp1}
%  \tilde{f}_\tau'(\x_{\tau+1})\geq \tilde{f}_\tau'(\x_{\tau+1}')+\frac{\tau+1}{2\tau}\|\x_{\tau+1}-\x_{\tau+1}'\|^2.
%\end{equation}
%Adding \eqref{eq:sens_opt_r} and \eqref{eq:sens_opt_rp1}, we get:
%$$\|\x_{\tau+1}-\x_{\tau+1}'\|^2\leq \frac{1}{\tau+1}|f_\tau(\x_{\tau+1}')+f_\tau'(\x_{\tau+1})-f_\tau(\x_{\tau+1})-f_\tau'(\x_{\tau+1}')|\leq \frac{2L}{\tau+1}\|\x_{\tau+1}-\x_{\tau+1}'\|.$$
%Lemma now follows using simplification. 
%\item {\bf $F-F'<\{f_i\},\ i<\tau$}: Define $\tilde{f}_\tau'(\x)=\frac{1}{2}\|\x-\hatx_\tau'\|^2+\eta_\tau f_\tau(\x)$ and let $\x_{\tau+1}'=\argmin_{\x\in \C} \tilde{f}_\tau'(\x)$. Then, similar to \eqref{eq:sens_opt_r}, we get:
%\begin{equation}
%  \label{eq:sens_opt_rp1}
%  \tilde{f}_\tau'(\x_{\tau+1})\geq \tilde{f}_\tau'(\x_{\tau+1}')+\frac{\tau+1}{2\tau}\|\x_{\tau+1}-\x_{\tau+1}'\|^2.
%\end{equation}
%Adding \eqref{eq:sens_opt_r} and \eqref{eq:sens_opt_rp1}, we get:
%$$\|\x_{\tau+1}-\x_{\tau+1}'\|^2\leq \frac{\tau}{\tau+1}|(\x_{\tau+1}-\x_{\tau+1}')\cdot(\x_\tau-\x_\tau')|\leq \frac{\tau}{\tau+1}\|\x_{\tau+1}-\x_{\tau+1}'\|\|\x_{\tau}-\x_{\tau}'\|.$$
%Lemma now follows after simplification and using induction hypothesis. 
%\end{itemize}
%\end{proof}
The above lemma shows that changing one function in $F$ can lead to a change of at most $2L/t$ in our $t$-th iterate. Hence, intuitively, adding a noise of the same order should make the $t$-th step of the algorithm differentially private. We make the claim precise in the following lemma. 
\begin{lemma}
Let $c>0$ be a constant, $T=|F|>0$ be the total number of iterations, and $\beta=\\ \frac{2L T^{0.5+c}}{t}\sqrt{\frac{2}{\epsilon}\left(\ln\frac{T}{\delta}+\frac{\sqrt{\epsilon}}{T^{0.5+c}}\right)}$, where $L$ is the maximum Lipschitz constant of any function in the function sequence $F$. Then step $t$ of algorithm~\ref{alg:igd} is $(\frac{\sqrt\epsilon}{T^{0.5+c}},\frac{\delta}{T})$-differentially private.
\label{Lem:SingGenPriv_igd}
\end{lemma}
See Section \ref{sec:OCPPriv} for the proof. Note that the proof in Section \ref{sec:OCPPriv} is for a generalized class of OCP (see Section \ref{sec:OCP} below). Setting $\lambda_\A=2L$ in the proof of Lemma \ref{Lem:SingGenPriv}, we get the proof of Lemma \ref{Lem:SingGenPriv_igd} above.

Now, the above lemma shows $(\frac{\sqrt\epsilon}{T^{0.5+c}},\frac{\delta}{T})$-differential privacy for each step. Hence, using a simple composition argument (see \cite{DL}) should guarantee $(T^{0.5-c}\epsilon, \delta)$-differential privacy. So to get a constant $\epsilon$ privacy, we will need $c=0.5$. That is, a noise of the order $O(T/t)$ needs to be added at each step, which intuitively means that the noise added is larger than the effect of incoming function $f_t$ and hence can lead to an arbitrary bad regret. 

To avoid this problem, we need to exploit the interdependence between the iterates (and outputs) of our algorithm so as to obtain a better bound than the one obtained by using the union bound. For this purpose, we use an interesting lemma by \cite{DRV} that bounds relative entropy of two random variables in terms of $L_\infty$ norm of their probability density ratio and also a proof technique developed by \cite{HR,HLM} for the problem of releasing differentially private databases. See Section \ref{sec:OCPPriv} for details. 
%Our proof technique is inspired by \cite{HR}. 

Now, we state our privacy theorem for the private \igd\ algorithm (Algorithm~\ref{alg:igd}) when it is executed for $T$-iterations.
\begin{thm}[Privacy]
%If $c\geq\frac{\ln\frac{1}{2}\ln\frac{2}{\delta}}{2\ln T}$, 
Algorithm~\ref{alg:igd} is $(3\epsilon,2\delta)$-differentially private.
\label{Thm:GenPri_igd}
\end{thm}
See Section \ref{sec:OCPPriv} (Theorem \ref{Thm:GenPri}) for a detailed proof. Although the proof in Theorem \ref{Thm:GenPri} is for a general class of OCP (see Section \ref{sec:OCP} below), the same proof holds for Theorem \ref{Thm:GenPri_igd} above. 

Having provided the privacy guarantee, we now prove that the noise added by our algorithm doesn't affect the regret arbitrarily and that its regret is still bounded by $\tilde O(\sqrt{T})$. 
\begin{thm}[Regret bound]
Let $L$ be the maximum Lipschitz constant and let $\alpha$ be the minimum strong convexity parameter of any function $f_t$ in the function sequence $F$. Then the expected regret of the private \igd\ algorithm over $T$-time steps is $\tilde O(\sqrt{T})$. Specifically, 
$$\E[\sum_{t=1}^Tf_t(\hat\x_t)]-\min_{\x\in\C}\sum_{t=1}^Tf_t(\x))\leq C\left(\frac{L^2d\ln^{1.5} \frac{T}{\delta}}{\alpha\sqrt{\epsilon}}\sqrt{T}\right),$$%\log T+\frac{2L^2 \sqrt{T\ln\sqrt{\frac{2}{\delta}}}}{\alpha}\sqrt{\frac{2}{\epsilon}\left(\ln\frac{T}{\delta}+\frac{\sqrt{\epsilon}}{\sqrt{T\ln\sqrt{\frac{2}{\delta}}}}\right)}\left(\frac{\sqrt{2}\Gamma((p+1)/2)\ln n}{\Gamma(p/2)}\right)$$
where $C>0$ is a constant and $d$ is the dimensionality of the output space. 
\label{thm:util_igd}
\end{thm}  
See Section \ref{sec:OCPReg} (Theorem \ref{thm:util}) for the proof.  Although the proof in Theorem \ref{thm:util} is for a general class of OCP (see Section \ref{sec:OCP} below), the same proof holds for Theorem \ref{thm:util_igd} above when combined with the regret bound for non-private \igd\, by \cite{KB10} (Theorem 4.5). 
%\subsubsection{Efficiency issues}
%%%\vspace*{-7pt}
\subsection{General Framework}
%%%\vspace*{-7pt}
\label{sec:OCP}
%In the previous section, we utilized the sensitivity bound (see Lemma~\ref{lemma:sens_igd}) and regret bound of \igd\ to show that a simple output perturbation based algorithm provides differential privacy along with bounded regret. 
In the previous section, we showed that a simple output perturbation to the \igd\ updates can be shown to have bounded regret while preserving differential privacy. In this section, we generalize our approach  to provide privacy as well as regret guarantees for any \ocp\ algorithm that satisfies certain criteria discussed below. %An \ocp\ algorithm takes the function sequence $F_t=\langle f_1, \dots, f_t\rangle$ and the previous iterates $X_t=\langle \x_1, \dots, \x_t\rangle$ to output a new iterate $\x_{t+1}\in \C$ so that the total loss $\sum_t f_t(\x_t)$ is minimized. 

Recall that, for a differentially private \ocp\ algorithm we need that with high probability, an algorithm should not produce a {\it significantly} different output for a {\it slightly} different function sequence $F_t'$. To formalize this notion, we defined sensitivity in the previous section (see Definition~\ref{defn:sensitivity}). Now, if the sensitivity of an algorithm to a single change in the function sequence $F$ doesn't decrease with $t$, then we might add noise larger than the effect of the function, hence providing poor regret.  

Another natural requirement for the \ocp\ algorithm is that it should have a provably low regret bound. There exists a variety of methods in literature which satisfy this requirement up to different degrees depending on the class of the functions $f_t$. 

Assuming that an \ocp\ algorithm satisfies the above two specified requirements, \ie its $L_2$ sensitivity (see Definition~\ref{defn:sensitivity}) and its regret is bounded, we provide a general framework for adapting the given \ocp\ algorithm into a differentially private algorithm. Formally, the given \ocp\ algorithm $\A$ should satisfy the following two conditions:
\begin{itemize}
\item $L_2$-sensitivity: The $L_2$-sensitivity (${\mathcal S}(\A)$) of the algorithm $\A$ should decay linearly with the time steps, \ie 
\begin{equation}
{\mathcal S}(\A)\leq \frac{\lambda_\A}{t},
\label{eq:sens_ocp}
\end{equation}
where $\lambda_\A>0$ is a constant depending only on $\A$, strong convexity, and Lipschitz constant of the functions in $F$. 
\item Regret bound $\R_{\A}(T)$: The regret of the algorithm is assumed to be bounded, typically by a sub-linear function of $T$. 
\end{itemize}
Given $\A$, we convert it into a private algorithm by perturbing $\x_{t+1}$ (output of $\A$ at $t$-th step) by a small amount of noise, whose magnitude is dependent on the sensitivity parameter $\lambda_\A$ of $\A$, and output its projection back onto the set $\C$. Note that, our Private \ocp\ algorithm also stores the ``uncorrupted'' iterate $\x_{t+1}$, as it would be used in the next step. See Algorithm~\ref{alg:ocp_diff} for a pseudo-code of our method. Now, using techniques similar to the ones described in the previous section, we obtain both privacy and regret bound for our Private \ocp\ algorithm. See Section \ref{Sec:OCP1} for detailed analysis of our privacy guarantee and the regret bound. 

In Section~\ref{sec:IGD}, we demonstrated the use of our \emph{abstract} private \ocp\ framework to convert \igd\ algorithm into a private \ocp\ method. Furthermore, in Sections \ref{sec:FTL} and \ref{sec:GIGA} we show two more applications of this technique to produce private FTL and private GIGA algorithm respectively. Similar to \igd, the privacy and regret bounds for these two algorithms follow almost immediately from the guarantees of our \ocp\ framework once the sensitivity bounds are established.

Here, we would like to note that \igd\ has better sensitivity guarantees than GIGA as \igd\ requires only Lipschitz continuity as against Lipschitz continuity of the gradient required by GIGA. Also, \igd\ is more efficient than FTL. Hence, for general strongly convex, Lipschitz continuous functions, \igd\ should be the private algorithm of choice for a given \ocp\  problem.
\begin{algorithm}[tb]
	\caption{Private \ocp\ Method (POCP)}
	\begin{algorithmic}[1]
		\STATE {\bfseries Input:} \ocp\ algorithm $\A$, cost function sequence $F=\langle f_1,\cdots,f_T\rangle$ and the convex set $\C$
                \STATE {\bfseries Parameter:} privacy parameters $(\epsilon, \delta)$
		\STATE Choose $\x_1$ and $\hat\x_1$ randomly from $\C$
		\FOR{$t=1$ to $T-1$} 
                \STATE \textbf{Cost:} $\ \ L_t(\hat\x_t)=f_t(\hat\x_t)$
                \STATE \textbf{\ocp\ Update:} $\ \ \x_{t+1}\leftarrow \A(\langle f_1, \dots, f_t \rangle, \langle\x_1, \dots, \x_t \rangle, \C)$
                \STATE \textbf{Noise Addition:} $\ \ \tx_{t+1}\leftarrow \x_{t+1}+\b$,\ \ $\b\sim\mathcal{N}(0^d,\frac{\beta^2}{t^2}\I^d )$, where  \ $\beta= \lambda_\A T^{0.5+c} \sqrt{\frac{2}{\epsilon}\left(\ln\frac{T}{\delta}+\frac{\sqrt{\epsilon}}{T^{0.5+c}}\right)}$  and $c=\frac{\ln\frac{1}{2}\ln(2/\delta)}{2\ln T}$
                %\STATE \textbf{Noise Addition:} $\hat\x_{t+1}\leftarrow \argmin_{\x\in \C}\left(\|\x-\x_{t+1}-b\|^2\right),\ \ 
                \STATE Output $\hat\x_{t+1}=\argmin_{\x\in \C}\left(\|\x-\tx_{t+1}\|_2^2\right)$
		\ENDFOR					
	\end{algorithmic}
	\label{alg:ocp_diff}
%%\vspace*{-2pt}
\end{algorithm}
\subsection{Privacy Guarantee for Private Online Convex Programming}
\label{Sec:OCP1}
\label{sec:OCPPriv}
Note that every step of our private algorithm adds noise proportional to the sensitivity of the algorithm at that step to obfuscate the output, so as to provide privacy guarantee for that particular step. We make the claim precise in the following lemma. 
\begin{lemma}
Let $c>0$ be any constant, and $\beta=\lambda_\A T^{0.5+c}\sqrt{\frac{2}{\epsilon}\left(\ln\frac{T}{\delta}+\frac{\sqrt{\epsilon}}{T^{0.5+c}}\right)}$. Then step $t$ of algorithm~\ref{alg:ocp_diff}, i.e., $t$-th step output $\hatx_{t+1}$ is $(\frac{\sqrt\epsilon}{T^{0.5+c}},\frac{\delta}{T})$-differentially private.
\label{Lem:SingGenPriv}
\end{lemma}

\begin{proof}
As the output $\hatx_{t+1}$ is just a projection, i.e., a function (independent of the input functions $F$) of $\tx_{t+1}$, hence $(\epsilon, \delta)$-differential privacy for $\tx_{t+1}$ would imply the same for $\hatx_{t+1}$.
 
Now by the definition of differential privacy (see Definition~\ref{def:dp}), $\txt$ is $(\epsilon_1, \frac{\delta}{T})$-differential private, if for any measurable set $\Omega\subseteq\mathbb{R}^{p}$:
$$\Pr[\txt\in \Omega]\leq e^{\epsilon_1}\Pr[\txt'\in \Omega]+\delta/T,$$
where $\txt=\xt+b$ is the output of the noise additions step (see Algorithm~\ref{alg:ocp_diff}, Step 7) of our differentially private algorithm $\A_P$, when applied to function sequence $F_t=\langle f_1, \dots, f_t\rangle$. Similarly, $\txt'=\xt'+b$ is the output of the noise addition to $\xt'$ which is obtained by applying update step to $F_t'$ where $F_t'$ differs from $F_t$ in exactly one function entry. 

Now, $\txt\sim {\mathcal N}(\x_{t+1},\frac{\beta^2}{t^2} \mathbb{I}^d)$ and $\txt'\sim {\mathcal N}(\x_{t+1}', \frac{\beta^2}{t^2} \mathbb{I}^d)$. Hence:
\begin{eqnarray*}
\frac{\Pr[\txt\in \Omega]}{\Pr[\txt'\in \Omega]}=\frac{\int_{\x\in \Omega}\pdf(\txt=\x)}{\int_{\x\in \Omega}\pdf(\txt'=\x)}=\frac{\int_{\x\in \Omega}\exp\left(-\frac{\ltwo{\x-\xt}^2}{2\frac{\beta^2}{t^2}}\right)d\x}{\int_{\x\in \Omega}\exp\left(-\frac{\ltwo{\x-\xt'}^2}{2\frac{\beta^2}{t^2}}\right)d\x}
\end{eqnarray*}
%Let $b=\theta-\mathcal{M}_i(T_i)$, and $f=\mathcal{M}_i(T'_i)-\mathcal{M}_i(T_i)$. We have


Let $\dxt=\xt-\xt'$. Next, we bound each individual term in the above integration: 
\begin{align}
  \frac{\exp\left(-\frac{t^2 \ltwo{\x-\xt}^2}{2\beta^2}\right)}{\exp\left(-\frac{t^2\ltwo{\x-\xt'}^2}{2\beta^2}\right)}&=\exp\left(\frac{t^2}{2\beta^2}\dxt^T(2\x-\xt-\xt')\right),\nonumber\\
&=\exp\left(\frac{t^2}{2 \beta^2}\left(2\dxt^T(\x-\xt)-\|\dxt\|_2^2\right)\right), \nonumber\\
&\leq \exp\left(\frac{t^2}{2 \beta^2 }\left(2|\dxt^T(\x-\xt)|+\|\dxt\|_2^2\right)\right), \nonumber\\
&\leq \exp\left(\frac{t^2}{\beta^2}|\dxt^T(\x-\xt)|\right)\exp\left(\frac{\lambda_\A^2}{2\beta^2}\right), 
\label{eq:HPB}
\end{align}
where the last inequality follows from the sensitivity assumption~\eqref{eq:sens_ocp}. 

Since $\txt\sim\mathcal{N}(\xt,\frac{\beta^2}{t^2}\I_p)$, we have $(\txt-\xt)^T\dxt\sim\mathcal{N}(0,\frac{\beta^2}{t^2}\|\dxt\|_2^2)$. %Using the maximum value of $f$ (from the assumption on the sensitivity of $\mathcal{A}(T_i))$, we analyze the worst case,~\emph{i.e.,} we assume $\langle b,f\rangle\sim\mathcal{N}(0,\frac{\beta^2\lambda^2}{i^2})$. 
Now, using \eqref{eq:sens_ocp} and Mill's inequality, $$\Pr[|(\txt-\xt)^T\dxt|\geq \frac{\beta\lambda_\A}{t^2}z]\leq \Pr[|(\txt-\xt)^T(\dxt)|\geq\frac{\beta}{t}\|\xt-\xt'\|z]\leq e^{-\frac{z^2}{2}},$$ where $z>0$. Setting R.H.S. $\leq\frac{\delta}{T}$, we have $z\geq\sqrt{2\ln\frac{T}{\delta}}$. 

We call the set of $\txt\in \Omega$ to be the ``good set'' $\G$ if 
\begin{equation}
\label{eq:good}
(\txt-\xt)^T\dxt\geq\frac{\beta\lambda_\A}{t^2}z.
\end{equation}
Using the above bound, $\Pr[\txt\not\in \G]\leq \frac{\delta}{T}$ and for all $\x\in \G$:
\begin{align}
\exp\left(\frac{t^2}{\beta^2}|\dxt^T(\x-\xt)|\right)\exp\left(\frac{\lambda_\A^2}{2\beta^2}\right)&\leq \exp\left(\frac{\lambda_\A^2}{2\beta^2}+\frac{\lambda_\A}{\beta}\sqrt{2\ln\frac{T}{\delta}}\right),\nonumber\\
&\leq e^{\epsilon_1},
\label{eq:expupg}
\end{align}
where $\epsilon_1=\frac{\sqrt\epsilon}{T^{0.5+c}}$ and $\beta$ is as given in the Lemma statement. 

Similarly, we can define set $\G'$ for $\txt'$ and furthermore, 
\begin{equation}
  \label{eq:gg}
  \Pr[\txt\in\G]=\Pr[\txt'\in \G'].
\end{equation}
Combining \eqref{eq:HPB} and \eqref{eq:expupg}:
\begin{equation}
  \label{eq:ogog}
  \Pr[\txt\in\Omega|\txt\in \G]\leq e^{\epsilon_1}\Pr[\txt'\in \Omega|\txt'\in \G'].
\end{equation}
Using \eqref{eq:gg} and \eqref{eq:ogog}:
\begin{align}
  \Pr[\txt\in \Omega]&\leq \Pr[\txt\in \Omega|\txt\in \G]\Pr[\txt\in \G]+\Pr[\txt\not\in \G],\nonumber\\
& \leq e^{\epsilon_1} \Pr[\txt'\in \Omega|\txt\in \G]\Pr[\txt'\in \G]+\delta, \nonumber\\
& \leq e^{\epsilon_1} \Pr[\txt'\in \Omega]+\delta. 
\label{eq:txtx}
\end{align}
Hence, proved. 
\end{proof}

The above lemma shows $(\frac{\sqrt\epsilon}{T^{0.5+c}},\frac{\delta}{T})$-differential privacy for each step of the \ocp\ algorithm. To prove the privacy of our online Algorithm \ref{alg:ocp_diff} over {\em all} $T$-iterations we use the following lemma by \cite{DRV}. Our proof strategy from here on is inspired from a proof technique developed by \cite{HR}. 

\begin{lemma}[\cite{DRV}]
Suppose two random variables $Y$ and $Z$ satisfy $$D_\infty(Y||Z)=\max_{w\in\supp(Y)}\ln\left(\frac{\pdf[Y=w]}{\pdf[Z=w]}\right)\leq\epsilon,\ \ \ D_{\infty}(Z||Y)\leq\epsilon.$$ Then $D(Y||Z)=\int_{w\in\supp(Y)}\pdf[Y=w]\ln\left(\frac{\pdf[Y=w]}{\pdf[Z=w]}\right)\leq 2\epsilon^2$. Here $supp(Y)$ is the support set of a random variable $Y$.
\label{lem:Dwork}
\end{lemma}

We now state a technical lemma which will be useful for our privacy. 

\begin{lemma}
Assuming that at each stage $T$,  algorithm~\ref{alg:ocp_diff} preserves $\frac{\sqrt{\epsilon}}{T^{0.5+c}}$-differential privacy, $$\E_{ \txt}\left[\ln\left(\frac{\pdf[\txt]}{\pdf[\txt'=\txt]}\right)\right]\leq\frac{2\epsilon}{T^{1+2c}},$$
where $\txt$ and $\txt'$ are output of the $t$-th time step Noise Addition Step of our private ocp\ algorithm (Algorithm~\ref{alg:ocp_diff}), when applied to function sequences $F_t$ and $F_t'$ differing in exactly one function entry. 
\label{lem:pro}
\end{lemma}
\begin{proof}
Using the fact that $\txt$ is $\frac{\sqrt{\epsilon}}{T^{0.5+c}}$-differential private: 
$$\forall \x,\hspace{0.1cm}-\frac{\sqrt{\epsilon}}{T^{0.5+c}}\leq\ln\left(\frac{\pdf[\txt=\x]}{\pdf[\txt'=\x]}\right)\leq \frac{\sqrt{\epsilon}}{T^{0.5+c}}.$$
Lemma now follows using the above observation with Lemma~\ref{lem:Dwork}. 
\end{proof}
 
Finally, we state the privacy guarantee for algorithm~\ref{alg:ocp_diff} over all the $T$-iterations.
\begin{thm}[Privacy \ocp]
The Private \ocp\ algorithm (see Algorithm~\ref{alg:ocp_diff}) is $(3\epsilon,2\delta)$-differentially private.
\label{Thm:GenPri}
\end{thm}

\begin{proof}
Following the notation from the proof of lemma~\ref{Lem:SingGenPriv} we define the ``good'' set $\G$ (see \eqref{eq:good}). Now, using \eqref{eq:gg} and Lemma~\ref{Lem:SingGenPriv}, for each round, 
\begin{equation}
\Pr[\txt\in\G]=\Pr[\txt'\in \G']=\frac{\delta}{T}.   
\end{equation}
Now, probability that the noise vector $\b=\txt-\xt=\txt'-\xt'$ always leads to ``good'' set in all $T$ rounds is $T\cdot \frac{\delta}{T}=\delta$. 

Now, we condition the remaining proof on the fact that the noise vector $\b$ in each round is such that $\tx_t\in \G$ and $\tx_t'\in \G'$. 

Let $L(\tx_1,\cdots,\tx_T)=\sum_{t=1}^T\ln\left(\frac{\pdf(\tx_t)}{\pdf(\tx_t'=\tx_t)}\right)$, where each $\x_t\in\mathbb{R}^d$.

Therefore, by Lemma~\ref{lem:pro}, $$\E[L(\tx_1,\cdots,\tx_T)]=\sum_{t=1}^T \E_{\tx_t}\left[\ln\left(\frac{\pdf(\tx_t)}{\pdf(\tx_t'=\tx_t)}\right)\right]\leq \frac{2T\epsilon}{T^{1+2c}}\leq\frac{2\epsilon}{T^{2c}}\leq 2\epsilon.$$

Let $Z_t=\ln\left(\frac{\pdf(\tilde{x}_t=\xt)}{\pdf(\tilde{x}_t'=\x_t)}\right)$. Since the randomness is freshly added in each iteration, $Z_t$ are independent. We have $L(\x_1,\cdots,\x_T)=\sum_{t=1}^T Z_t$, where $|Z_t|\leq\frac{\sqrt{\epsilon}}{T^{0.5+c}}$. By Azuma-Hoeffding's inequality
\begin{align*}
\Pr[L(\tx_1,\cdot,\tx_T)\geq 2\epsilon+\epsilon]&\leq 2\exp\left(\frac{-2\epsilon^2}{T\times\frac{\epsilon}{T^{1+2c}}}\right),\\
&\leq 2\exp\left(-2T^{2c}\right).
\end{align*}
Let $\delta=2\exp\left(-2T^{2c}\right)$. We have $-2T^{2c}=\ln\frac{\delta}{2}$. Solving for $c$ we get $c=\frac{(\ln (\frac{1}{2}\ln \frac{2}{\delta} )}{2\ln T}$.

Hence, with probability $1-\delta$, $3\epsilon$-differential privacy holds conditioned on $\tx_t\in\G$ and $\tx_t'\in\G'$, i.e, 
$$\forall\x, \hspace{0.1cm}\Pi_{t=1}^T\pdf(\x_t=\x)\leq e^{3\epsilon}\Pi_{t=1}^T\pdf(\tx_t'=\x).$$
Also, recall that with probability $1-\delta$, our noise vector $\b$ in each round itself was such that $\tx_t\in \G$ and $\tx_t'\in \G'$. Theorem now follows using an argument similar to \eqref{eq:txtx}. 
\end{proof}


\subsection{Generic Regret Bound Analysis for OCP}
\label{sec:OCPReg}
In this section, we provide a generic regret bound analysis for Algorithm \ref{alg:ocp_diff}. The regret of our private \ocp\ algorithm depends on the regret $\R_\A(T)$ the non-private learning algorithm $\A$.

\begin{thm}[Regret Bound]
Let $L>0$ be the maximum Lipschitz constant of any function $f_t$ in the sequence $F$, %and let $\alpha>0$ be the minimum strong convexity parameter of any function $f_t$ in $F$. 
 and let the regret of the non-private \ocp\ algorithm $\A$ over $T$-time steps is $\R_{\A}(T)$ and let $\lambda_\A$ be the sensitivity parameter of $\A$ (see \eqref{eq:sens_ocp}), then the expected regret of our Private \ocp\ algorithm (Algorithm~\ref{alg:ocp_diff}) follows:
$$\E\left[\sum_{t=1}^Tf_t(\hat\x_t)\right]-\min_{\x\in\C}\sum_{t=1}^Tf_t(\x)\leq 2dL\lambda_\A\sqrt{T}\frac{\ln^2\frac{T}{\delta}}{\sqrt{\epsilon}}+\R_{\A}(T),$$  
%is upper bounded by 
%$$\R_{\A}(T)+\lambda_\A \sqrt{T\ln\sqrt{\frac{2}{\delta}}}\sqrt{\frac{2}{\epsilon}\left(\ln\frac{T}{\delta}+\frac{\sqrt{\epsilon}}{\sqrt{T\ln\sqrt{\frac{2}{\delta}}}}\right)}\left(\frac{\sqrt{2}\Gamma((d+1)/2)\ln T}{\Gamma(d/2)}\right),$$
where $d$ is the dimensionality of the output space. That is, the regret bound is $ R_\A(T)+\tilde{O}\left(d\sqrt{T}\right)$. 
\label{thm:util}
\end{thm}  

\begin{proof}
Let $\hat\x_1,\cdots,\hat  \x_T$ be the output of the POCP algorithm~\ref{alg:ocp_diff}. By the Lipschitz continuity of the cost functions $f_t$ we have
\begin{eqnarray}
&&\sum_{t = 1}^T f_t(\hat{\x}_t)-\min_{\x\in\C}\sum_{t=1}^Tf_t(\x) \leq \sum_{t = 1}^T f_t(\x_t)-\min_{\x\in\C}\sum_{t=1}^Tf_t(\x) + L \sum_{t = 1 }^T \ltwo{\hat{\x}_t - \x_t}\\
&&= R_\A(T) +  L \sum_{t = 1 }^T \ltwo{\hat{\x}_t - \x_t}.
\label{eq:rahx}
\end{eqnarray}
Since at any time $t$,  $\hat\x_{t}$ is the projection of $\tilde\x_{t}$ on the convex set $\C$, we have $$\ltwo{\x_t-\hat\x_t}\leq\ltwo{\x_t-\tilde{\x}_t}=\ltwo{\b_t},$$ where $\b_t$ is the noise vector added at in the $t^{th}$ iteration of algorithm~\ref{alg:ocp_diff}. Therefore,
\begin{equation} 
\sum_{t=1}^T L \ltwo{\x_{t}-\hat\x_{t}}\leq L \sum_{t =1}^T\ltwo{\b_{t}}.
\label{eq:hxb}
\end{equation}
Now, $\b_{t} \sim \mathcal{N} ( \0^d, \frac{\beta^2}{t^2} \I^d) $ where $$\beta= \lambda_{\A}T^{0.5+c}\sqrt{\frac{2}{\epsilon}\left(\ln\frac{T}{\delta}+\frac{\sqrt{\epsilon}}{T^{0.5+c}}\right)}.$$
 
Therefore, $\ltwo{\b_{t}}$ follows Chi-distribution with parameters $\mu=\frac{\sqrt{2}\frac{\beta}{t} \Gamma((d+1)/2)}{\Gamma(d/2)}$ and $\sigma^2=\frac{\beta^2}{t^2}(d-\mu^2)$. 

Using $c = \frac{\ln{ (\frac{1}{2}\ln{\frac{2}{\delta}})} }{2\ln{T}}$,
\begin{align}
 \E[\sum_{\tau=1}^T\ltwo{\b_{\tau}}] &\leq \frac{\sqrt{2}\beta \Gamma((d+1)/2)}{\Gamma(d/2)} \int_{\tau =1}^T \frac{1}{t}d\tau, \nonumber\\
&= \frac{\Gamma((d+1)/2)}{\Gamma(d/2)} \lambda_\A\sqrt{T}\ln {T}\sqrt{\frac{2}{\epsilon}\ln{\frac{2}{\delta}}\left(\ln\frac{T}{\delta}+\frac{\sqrt{\epsilon}}{\sqrt{\frac{T}{2}\ln{\frac{2}{\delta}}}}\right)},\nonumber\\
&\leq 2d\lambda_\A\sqrt{T}\frac{\ln^2\frac{T}{\delta}}{\sqrt{\epsilon}}. 
\label{eq:noisenorm}
\end{align}
The theorem now follows by combining \eqref{eq:rahx}, \eqref{eq:hxb}, \eqref{eq:noisenorm}. 
\end{proof}
\subsection{Follow the Leader}
\label{sec:FTL}
As a specific instantiation of Algorithm \ref{alg:ocp_diff} we describe our Private Follow The Leader Algorithm (\pftl). It is based on the Follow The Leader algorithm (\ftl\,) by \cite{HKKA}. \ftl\, at each time step $t+1$ outputs $\x_{t+1}=\argmin_{\x\in\C}\frac{1}{t}\sum_{\tau=1}^t f_{\tau}(\x)$. The first vector $\x_1\in\C$ is chosen  arbitrarily without querying the data set.  For \pftl\ we instantiate the non-private algorithm $\A$ (in Algorithm \ref{alg:ocp_diff}) with the following. Let $\mathcal{A}(F_t)=\argmin_{\x\in\C}\frac{1}{t}\sum_{\tau =1}^t f_{\tau}(\x)$, where $F_t=\langle f_1,\cdots,f_t\rangle$. We assume the following regarding the cost functions. 
\begin{enumerate}
	\item The cost function $f_t(\x)$ can be written as $g_t(\langle \bm v_t,\x\rangle)+\frac{\alpha}{2}\ltwo{\x}^2$, where $g_t:\mathbb{R}\rightarrow\mathbb{R}$ is a univariate function and $\bm v_t$ is a vector s.t. $\ltwo{\bm v_t}\leq R$ (a constant). We need this condition for our regret bound.
	\item The cost function $f_t(\x)$ is $L$-Lipschitz in $\x$,~\emph{i.e.,} $|f_t(\x_1)-f_t(\x_2)|\leq L\ltwo{\x_1-\x_2},\forall \x_1,\x_2\in \C$.
	\item A relatively mild assumption is that the \emph{origin} ($\0^d$) is contained in the convex set $\C$.
\end{enumerate}

Our first lemma is about bounding the sensitivity of $\mathcal{A}(F_t)$.

\begin{lemma}
$L_2$-sensitivity of $\x_{t+1}=\argmin_{\x\in\C}\frac{1}{t}\sum_{\tau =1}^t f_{\tau}(\x)$ is $\frac{2L}{t\alpha}$.
\end{lemma}

\begin{proof}
$\x_{t+1}=\arg\min_{\x\in\C}\frac{1}{t}\sum_{\tau =1}^t f_{\tau}(\x)$ is the result of a constrained convex optimization on the convex set $\C$. For the ease of representation let $G_{t}(\x)=\frac{1}{t}\sum_{\tau=1}^t f_{\tau}(\x)$ . Let $G_t'$ be another summation where $G_t$ and $G_t'$  differ in exactly one of it summands. Let $\x'_{t+1}\in\C$ be the vector that minimizes $G'_{t}$.

For all points $y\in\C$, the following are true,
\begin{enumerate}
	\item $\subg{G_{t}}(\x_{t+1})^T(y-\x_{t+1})\geq 0$
	\item $\subg{G'_{t}}(\x'_{t+1})^T(y-\x'_{t+1})\geq 0$
\end{enumerate}
where $\subg{}$ is any subgradient of the function $G_t$ or $G_{t'}$.
The cost functions  $f_t$ are assumed to be $\alpha$-strongly convex. Thus, both $G_{t}$ and $G'_{t}$ are $\alpha$-strongly convex.
Thus, we have
\begin{eqnarray*}
&&G_t(\x'_{t+1})\geq G_t(\x_{t+1})+\frac{\alpha}{2}\ltwo{\x'_{t+1}-\x_{t+1}}^2\\
&&G'_t(\x_{t+1})\geq G'_t(\x'_{t+1})+\frac{\alpha}{2}\ltwo{\x'_{t+1}-\x_{i+1}}^2\\
\end{eqnarray*}
Combining the above two equations we have,
$$\alpha\ltwo{\x'_{t+1}-\x_{t+1}}^2\leq (G_t(\x'_{t+1})-G'_t(\x'_{t+1}))+(G'_t(\x_{t+1})-G_t(\x_{t+1}))$$
Let the summands of $G_t$ and $G'_k$ differ at position $k$. Therefore, $G_t(\x'_{t+1})-G'_t(\x'_{t+1})=\frac{1}{t}(f_k(\x'_{t+1})-f'_k(\x'_{t+1}))$ and $G'_t(\x_{t+1})-G_t(\x_{t+1})=\frac{1}{t}(f'_k(\x_{t+1})-f'_k(\x_{t+1}))$.
where $f'_k$ is another function differing from $f_k$.
Hence,
\begin{eqnarray}
&&\alpha\ltwo{\x'_{t+1}-\x_{t+1}}^2\leq\frac{1}{t}\left(f_k(\x'_{t+1})-f'_k(\x'_{t+1})+f'_k(\x_{t+1})-f_k(\x_{t+1})\right)\\
&&\leq \frac{2L}{t}\ltwo{\x'_{t+1}-\x_{t+1}}
\end{eqnarray}
The last inequality follows from the Lipschitz property of the cost function $f_t$. 
Finally,
$$\ltwo{\x'_{t+1}-\x_{t+1}}\leq \frac{2L}{t\alpha}$$
\end{proof}

We fix $\lambda_\mathcal{A}=\frac{2L}{\alpha}$ in Algorithm~\ref{alg:ocp_diff} as the sensitivity parameter. 

\begin{corollary}[Privacy]
Private \ftl\, is $(3\epsilon,2\delta)$-differentially private.
\end{corollary}
The proof of this corollary follows directly from Theorem \ref{Thm:GenPri}.

Before we state the regret bound for \pftl, we state the following theorem bounding the regret for non-private \ftl\, (\ie when we do not add noise to the output).  The proof can be obtained (with minor modification) from the regret bound analysis of the version of \ftl\, by  \cite{HAS}. 

\begin{thm}[Regret bound for \ftl\,]
Assume that for all $t$, the function $f_t(x)$ can be written as $g_t(\langle v_t,\x\rangle)+\frac{\alpha}{2}\ltwo{\x}^2$ for a univariate convex function $g_t(\langle v_t,\x\rangle)$ and some vector $v_t\in\mathbb{R}^p$. Assume that for some $R,G >0$, we have $\ltwo{v_t}\leq R$ and for all $\x\in\C$, we have $| g'_t(\langle v_t,\x\rangle)|\leq G$ and $|g''_t(\langle v_t,\x\rangle)|\geq 0$. Also assume that the convex set $\C$ contains the origin. The  non-private \ftl\, over $T$ rounds has~\emph{regret}
$$\leq \frac{1}{\alpha}\left(G\ R+C\alpha\right)^2\ln T$$
where $C$ is the diameter of the convex set $\C$.
\label{Thm:UtilKalai}
\end{thm}

We now state the regret bound for \pftl. It follows as a corollary from Theorem~\ref{thm:util}.

\begin{corollary}[Regret bound for \pftl\,]
Suppose for all $t$, $f_t$ satisfies all the conditions in theorem  \ref{Thm:UtilKalai} Let the Lipschitz constant of $f_t$ for all $t$ be at most $L$. Then, the expected regret (\emph{i.e.,} $\E[\sum_{t=1}^Tf_t(\hat\x_t)]-\min_{\x\in\C}\sum_{t=1}^T f_t(\x))$  is upper bounded by 
$$\frac{1}{\alpha}\left(\left(G R+C\alpha\right)^2\ln T+4d L^2\sqrt{T}\frac{\ln^2\frac{2}{\delta}}{\sqrt \epsilon}\right)$$
where $C$ is the diameter of the convex set $\C$ and $d$ is the dimensionality of the output space.
\end{corollary}

\subsection{Private GIGA Algorithm}
\label{sec:GIGA}
In this section, we apply our general differential privacy framework to the Generalized Infinitesimal Gradient Ascent (\giga) algorithm \cite{Zin}, which is one of the most popular algorithm for \ocp. 

For the rest of this section, we assume that each of the function $f_t$ in the input function sequence $F$ are {\em differentiable}, Lipschitz continous gradient and strongly convex. Note that this is stricter requirement than our private \igd\ algorithm where we only require Lipschitz continuity of $f_t$. 

\giga\ is a simple extension of the classical projected gradient method to the \ocp\ problem. Specifically, iterates $\x_{t+1}$ are obtained by a projection onto the convex set $\C$ of gradient descent step $\x_t-\eta_t\grad f_t(\x_t)$ where $\eta_t=1/\alpha t$, and $\alpha$ is the minimum strong convexity parameter of any function $f_t$ in $F$.  
\begin{algorithm}[tb]
	\caption{Private \giga Algorithm}
	\begin{algorithmic}[1]
		\STATE {\bfseries Input:} \ocp\ algorithm $\A$, cost function sequence $F=\langle f_1,\cdots,f_T\rangle$ and the convex set $\C$,  $t_q=2L_G^2/\alpha^2$
                \STATE {\bfseries Parameter:} privacy parameters $(\epsilon, \delta)$
		\STATE Choose $\x_1, \dots, \x_{t_q-1}$ and $\hat\x_1, \dots, \hat\x_{t_q-1}$ randomly from $\C$ and incur a cost of $\sum_{t=1}^{t_q-1} f_t(\hat\x_t) = constant( w.r.t. $T$)$
		\FOR{$t=t_q$ to $T-1$} 
             %   \STATE \textbf{Cost:} $\ \ L_t(\hat\x_t)=f_t(\hat\x_t)$
                \STATE \text{Step Size:} $\eta_t=\frac{2}{\alpha t}$
                \STATE \textbf{\giga\ Update:} $\ \ \x_{t+1}\leftarrow \argmin_{x\in \C}\left(\|\x_t-\eta_t\grad f_t(\x_t)\|_2^2\right)$
                \STATE \textbf{Noise Addition:} $\ \ \tx_{t+1}\leftarrow \x_{t+1}+\b$,\ \ $\b\sim\mathcal{N}(\0^d,\frac{\beta^2}{t^2}\I^d )$, where  \ $\beta= 2G T^{0.5+c} \sqrt{\frac{2}{\epsilon}\left(\ln\frac{T}{\delta}+\frac{\sqrt{\epsilon}}{T^{0.5+c}}\right)}$ where $c=\frac{\ln\frac{1}{2}\ln(2/\delta)}{2\ln T}$
                %\STATE \textbf{Noise Addition:} $\hat\x_{t+1}\leftarrow \argmin_{\x\in \C}\left(\|\x-\x_{t+1}-b\|^2\right),\ \ 
                \STATE Output $\hat\x_{t+1}=\argmin_{\x\in \C}\left(\|\x-\tx_{t+1}\|_2^2\right)$
		\ENDFOR					
	\end{algorithmic}
	\label{alg:giga_diff}
\end{algorithm} 

As discussed in Section~\ref{sec:OCP}, we can provide a private version of the \giga\ algorithm  using our generic Private \ocp\ framework (See Algorithm~\ref{alg:ocp_diff}). Algorithm~\ref{alg:giga_diff} details the steps involved in Private \giga. It is important to note that Algorithm \ref{alg:giga_diff} has an additional step (Step 3) compared to private \ocp\, (Algoritm \ref{alg:ocp_diff}). This step is important for acieving the sensitivity bound in Lemma \ref{lemma:sens_giga} below.

Similar to \igd\, in Section \ref{sec:IGD}, we can prove the privacy and regret guarantees, using Theorem~\ref{Thm:GenPri} and Theorem~\ref{thm:util}, if we can show that \giga\ satisfies the sensitivity assumption mentioned in \eqref{eq:sens_ocp} and has bounded regret $\R_{\giga}(T)$, which was shown to be logarithmic (for strongly convex functions $f_t$) by \cite{HKKA}. %Specifically, 
%$$\R_{\giga}(T)= O(\log T).$$
Next, we show the sensitivity bound for \giga. 
\begin{lemma}[{\bf \giga\ Sensitivity}]
\label{lemma:sens_giga}
For each $1 \leq \tau \leq t$, let $f_t$  have a $L_G$-continuous gradient. Then, the sensitivity of the \giga\ algorithm is $\frac{2G}{\alpha t}$ for the $t$-th iterate for $1 \leq t \leq T$ where $G=\max_\tau \|\grad f_t(x)\|_2, \forall x\in \C$.
\end{lemma}
\begin{proof}
Let the $t$-th iterate when \giga\ is applied to $F$ and $F'$ be $\x_{t+1}$ and $\x_{t+1}'$, respectively. Using this notation, to prove the $L_2$ sensitivity of \giga, we need to show that:
$$\|\x_{t+1}-\x_{t+1}'\|\leq \frac{2G}{\alpha t}$$ % t\geq t_q=2L_G^2/\alpha^2$$
We prove the above inequality using mathematical induction. \\
{\bf Base Case ($1\leq t\leq t_q=L_G^2/\alpha+1$)}: As $\x_1, \dots, \x_{t_q}$ are selected randomly, their value doesn't depend on the underlying dataset. \\
{\bf Induction Step $t=\tau>L_G^2/\alpha+1$}: We consider two cases:
\begin{itemize}
\item {\bf $F-F'=\{f_\tau\}$}: Since the difference between $F$ and $F'$ is only the $\tau$-th function, hence $\x_\tau=\x_\tau'$. Also, as $\C$ is a convex set:
\begin{align}
\|\x_{\tau+1}-\x_{\tau+1}'\|_2&\leq \|(\x_\tau-\eta_\tau\grad f_\tau(\x_\tau))-(\x_\tau-\eta_\tau\grad f_\tau'(\x_\tau))\|_2,\nonumber\\
&=\eta_\tau\|\grad f_\tau(\x_\tau)-\grad f_\tau'(\x_\tau)\|_2,\nonumber\\
&\leq \frac{2G}{\alpha \tau}. \nonumber
\end{align}
Hence, lemma holds in this case. 
\item {\bf $F-F'=\{f_i\},\ i< \tau$}: Again using convexity of $\C$, we get:
\begin{align}
\|\x_{\tau+1}-\x_{\tau+1}'\|_2^2&\leq \|(\x_\tau-\eta_\tau\grad f_\tau(\x_\tau))-(\x_\tau'-\eta_\tau\grad f_\tau(\x_\tau'))\|_2^2,\nonumber\\
&=\|\x_\tau-\x_\tau'\|_2^2+\eta_\tau^2\|\grad f_\tau(\x_\tau)-\grad f_\tau(\x_\tau')\|^2_2-2\eta_\tau(\x_\tau-\x_\tau')^T(\grad f_\tau(\x_\tau)-\grad f_\tau(\x_\tau')),\nonumber\\
&\leq (1+\eta_\tau^2L_G^2)\|\x_\tau-\x_\tau'\|_2^2-2\eta_\tau(\x_\tau-\x_\tau')^T(\grad f_\tau(\x_\tau)-\grad f_\tau(\x_\tau')),
%&\leq \left(1+\frac{L^2}{\alpha^2\tau^2}\right)\cdot\frac{C^2}{(\tau-1)^2}-2\eta_\tau(\x_\tau-\x_\tau')^T(\grad f_\tau(\x_\tau)-\grad f_\tau(\x_\tau')),
\label{eq:gigaxxup}
\end{align}
where the last equation follows using Lipschitz continuity of $\grad f_t$. and the last equation follows using induction hypothesis. 

Also, using strong convexity:
$$(\x_\tau-\x_\tau')^T(\grad f_\tau(\x_\tau)-\grad f_\tau(\x_\tau'))\leq -\alpha\|\x_\tau-\x_\tau'\|_2^2.$$
Combining the above observation and the induction hypothesis with \eqref{eq:gigaxxup}:
\begin{align}
  \|\x_{\tau+1}-\x_{\tau+1}'\|_2^2&\leq \left(1+L_G^2\eta_\tau^2-2\alpha\eta_\tau\right)\cdot\frac{4G^2}{(\tau-1)^2}.
\end{align}
Lemma now follows by setting $\eta_\tau=\frac{2}{\alpha \tau}$ and $\tau>\frac{2L_G^2}{\alpha^2}$. 
\end{itemize}
\end{proof}
Using the above lemma and the regret bound for \giga\ from \cite{HKKA}(Theorem 1), along with Theorem~\ref{Thm:GenPri} and Theorem~\ref{thm:util}, we get the privacy guarantee and regret bound for our private \giga\ algorithm (Algorithm \ref{alg:giga_diff}). 

\begin{thm}
Let each $f_t$ for $1 \leq t \leq T$ have a $L_G$-continuous gradient. Let $G$ be the maximum norm of gradient of any function $f_t$ in $F$ and let $\alpha>0$ be the minimum strong convexity parameter for $f_t\in F$. Then, private \giga\ (see Algorithm~\ref{alg:giga_diff}) is $(3\epsilon, 2\delta)$-private and has the expected regret that satisfies
$$\E[\R_{PGIGA}(T)]\leq \frac{2G^2}{H}(1+\log T)+\frac{4dL_GG\sqrt{T}}{\alpha }\frac{\ln^2\frac{T}{\delta}}{\sqrt{\epsilon}}+\frac{2L_G^3\ltwo{\mathcal{C}}}{\alpha}$$
where $\ltwo{\mathcal{C}}$ is the diameter of the convex set $\mathcal{C}$ and $d$ is the dimensionality of the output space.
\end{thm}
\begin{proof}
Observe that we start the algorithm only after $t_q =\frac{2L_G^2}{\alpha^2}$ iterations. During this time, the algorithm incurs a worst case constant regret which appears as an additive term in the final regret of the algorithm at time $T$. For iterations $t \geq t_q$, the proof follows directly by using  Theorem~\ref{Thm:GenPri} and Theorem~\ref{thm:util}. Thus the regret just increases by a constant which has no asymptotic effect. Note that we use $\eta_t=2/\alpha t$, instead of $\eta_t=1/\alpha t$. This difference in the step size increases the regret of \giga\ as given by \cite{HKKA} by a factor of 2. 
\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "nips2011"
%%% End: 

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "nips2011"
%%% End: 

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "nips2011"
%%% End: 


==> method.tex <==
%\vspace*{-7pt}
\section{Method}
%\vspace*{-7pt}
In this section we first adapt the Implicit Gradient Descent method (\igd)\ \cite{KB10} to obtain a differentially private \ocp\ algorithm with provable sub-linear regret. We then generalize our approach to modify any \ocp\ algorithm that satisfies ``certain criteria'' to obtain a differentially private algorithm with sub-linear regret. Special cases of our approach include the Gradient Infinitesimal Gradient Ascent method (GIGA) \cite{Zin}, the Follow The Leader algorithm (FTL) \cite{HKKA}, and a special case of Dual Averaging Method (DA) \cite{xiao}. 

\input{lin.tex}
%\input{lin}
\input{logGuar}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "nips2011"
%%% End: 


==> partialSum.tex <==
\subsection{ FTL for Quadratic Costs} 
\label{sec:logRegret}
We prove the privacy and utility guarantees for our private FTL algorithm with Quadratic Cost functions here.
\begin{thm}
Let $f_t =\frac{1}{2} (y_t - \v_t^T\x)^2 + \frac{\alpha}{2}\ltwo{\x}^2$ for each $t$ be Lipschitz continuous with parameter $L$. For $\hat{\x}_t$  the output of the private FTL algorithm as in Algorithm \ref{Algo:quad} , and $\x_t$ the corresponding output of the non-private FTL, we have, with high probability,  $$\R_{privacy} = \sum_{t = 1 }^T ( f_t(\hat{\x}_t) - f_t(\x_t) ) = O( L^2 R^2d^2 \frac{1}{\sqrt{\epsilon}} \log^{1.5}{T} \log{\sqrt{\frac{\log{T}}{\delta}}} ) $$ 
\end{thm}
\begin{proof}
Using Lipschitz continuity of functions $f_1,\dots, f_t$ , 
\begin{align}
\R_{privacy} =  \sum_{t = 1} ^{T} ( f_t(\hat{\x}_t) - f_t(\x_t) )\leq L \sum_{t = 1} ^{T}  \ltwo{\hat{\x}_{t+1} - \x_{t+1} }   \label{eqnpriv}
\end{align}
We now bound $ \ltwo{\hat{\x}_{t+1} - \x_{t+1} }$. Let $\hat{V}_t = V_t + A_t$ and $\hat{\K}_t = \K_t + \N_t$  where $A_t$ and $\N_t$ are the noise additions introduced by the Private Partial sum Computing algorithm \ref{Algo:partialSum}.

From the Update Equation \eqref{eqnref:QuadUpdate} we have
\begin{align}
(\hat{V}_{t} + t\alpha \I ) \hat{\x}_t =  \hat{K}_t\quad \Leftrightarrow\quad (\frac{1}{t}\hat{V}_{t} + \alpha \I )\hat{x}_t &= \frac{1}{t} \hat{\K}_t  \label{eqnprav1}
\end{align}
Similarly for the non-private FTL's update equation we have, 
\begin{align}
(\frac{1}{t} V_t + \alpha \I) \x_t &= \frac{1}{t}\K_t \label{eqnprav2}
\end{align}
By combining \eqref{eqnprav1} and \eqref{eqnprav2}, we get:

$$ (\frac{1}{t}\hat{V}_{t} + \alpha \I )( \hat{\x}_t -\x_t) = \frac{1}{t} \N_t - \frac{1}{t}A_t\x_t $$
By triangle inequality we have,
\begin{equation}
\ltwo{ (\frac{1}{t}\hat{V}_{t} + \alpha \I )( \hat{\x}_t -\x_t) }  \geq \ltwo{ (\frac{1}{t}V_{t} + \alpha \I )( \hat{\x}_t -\x_t) } - \ltwo {  \frac{1}{t} A_t( \hat{\x}_t -\x_t)  }
\label{eq:Afbcs1}
\end{equation}
Now, the spectral norm $\ltwo{A_t}$ of $A_t$ satisfies, $\ltwo{A_t} \leq \lfrob{A_t}$. Furthermore, using Cauchy Schwartz inequality:
 \begin{align}
\ltwo {  \frac{1}{t} A_t( \hat{\x}_t -\x_t)  } &\leq \frac{1}{t} \ltwo{A_t}\ltwo{\hat{\x}_t - \x_t } \leq  \frac{1}{t} \lfrob{A_t}\ltwo{\hat{\x}_t - \x_t }
\label{eq:Afbcs}
\end{align}
Thus by combining \eqref{eq:Afbcs1}, \eqref{eq:Afbcs} and using the fact that the spectral norm of $(\frac{1}{t}V_{t} + \alpha \I)$ is lower-bounded by $\alpha$, 
\begin{align}
 (\alpha - \frac{\lfrob{A_t}}{t} ) \ltwo{\hat{\x}_t - \x_t }&\leq  \frac{1}{t}\ltwo{ \N_t} + \frac{1}{t}\ltwo{A_t\x_t}\label{eq:Afbcs3}
\end{align}
Now, each entry of the matrix $A_t$ is drawn from $\mathcal{N}( 0, \sigma^2)$ for $\sigma^2 = \frac{R^2}{\epsilon}\log{T}\log{\frac{\log{T}}{\delta}}$. Thus the spectral norm of $A_t$, $\ltwo{A_t}$ is a sum of independent Gaussian random variables and itself follows the Gaussian distribution with the variance multiplied. Hence by definition,  $\lfrob{A_t}$ follows Chi distribution with mean $\mu = \frac{\sqrt{2}\sigma\Gamma{(d^2+1)/2}}{\Gamma({d^2/2})}$ and Variance $\sigma^2 ( d^2 - \mu^2)$. Thus, with high probability 
 %(replace with an exact value here ? ) 
  $$\lfrob{A_t} \leq \sqrt{2}\sigma d^2+ \sigma d.$$
 Similarly, $\ltwo{\N_t} \leq \sqrt{2}\sigma d + \sigma \sqrt{d} $. Also, $\x_t = (\frac{1}{t}V_t + \alpha \I^d)^{-1} K_t$ Thus $\ltwo{\x_t} \leq R$ Using the above observation with \eqref{eq:Afbcs3}, 
 \begin{align*}
 \ltwo{\hat{\x}_t - \x_t } &\leq  \frac{1}{t}\cdot\frac{\ltwo{ \N_t} + \ltwo{A_t\x_t}}{\alpha - \frac{\lfrob{A_t}R}{t}}\leq \frac{O(\sigma R d^2)}{t}. 
%\leq \frac{1}{t}\cdot\frac{2\sqrt{2}Rd + 2\sigma Rd}{\alpha}=
 \end{align*}
Summing the above equation over $t=1$ to $T$:
 \begin{align*}
 \sum_{\tau = 1}^t \ltwo{\hat{\x}_{t+1} - \x_{t+1} } \leq \int_{\tau = 1 }^{T} \frac{O(\sigma R d^2)}{\tau} d\tau= O(\sigma R d^2)\log{T}= O( R^2 d^2 \frac{1}{\sqrt{\epsilon}} (\log{T})^{1.5} \log{\sqrt{\frac{log{T}}{\delta}}} ).
 \end{align*}
 The result now follows by using the above bound with \eqref{eqnpriv}. 
\end{proof}

\subsection{ Computing Partial Sums Privately }
\label{sec:partialSum}

In this section we generalize a technique proposed in \cite{DNPR} to compute partial sums for real vectors arriving online when each vector belongs to a different party. Differential Privacy of the algorithm guarantees that under an adversarial modification of one of the vectors, the sums output by the algorithm remain {\it almost} invariant. Thus the adversary cannot extract information about any particular party from the output of the algorithm.We use this algorithm as a black box to guarantee the privacy of our QPFTL algorithm.

We begin this section with a brief description of the algorithm and then show the privacy guarantees. 

For simplification of exposition we assume that $T = 2^k$ for some positive integer $k$. We compute a binary tree $\B$ of partial sums with leaves as the input vectors arriving online. Each node in the tree represents the sum of the vectors in the subtree rooted at the node. To represent this, we label the node at some level $i$ with strings in $\{0,1\}^{i}$. (The root is labeled with the empty string $\empty$) A node labeled with a string $s$ of length $i$ represents the privately computed partial sum  

$$\hat{\B}_s = \sum_{\begin{subarray}{c}j: \text{string}(j)  = s\circ t\\ t \in \{0,1\}^{k-i}\end{subarray} } \uu_j$$ where string(j) is the bit string representation of $j$ in $\{0,1\}^k$ and $\circ$ is the concatenation operation on strings.

Note that for this technique to work, we need to know the number of arriving values, $T$ in advance. We create a node in the tree only when all the vectors that form the leaves of the subtree rooted at the node have arrived. At time instant $\tau$ we receive vector $u_{\tau}$ and create the nodes which can now be created bottom up. Whenever we add a node, we compute the value to be stored at the node by summing up the values at its two children and adding a Gaussian noise of $0$ mean and appropriately computed variance.

To output the partial sum at an instant $\tau$, we express the sum in the form of sum of values at nodes in the tree, where we choose the nodes at the higher levels first.
\begin{algorithm}
	\caption{Private Partial Sum($\{\uu_i\}$, $\epsilon$, $\delta$, $R \geq max_{i \leq T} \ltwo{\uu_i} $ ) }
	\begin{algorithmic}[1]
		\REQUIRE Data vectors $\uu_i$ arriving online, privacy parameters $\epsilon$ and $\delta$,  $R$, and dimension of the vectors $d$
		\STATE Set $ \sigma^2 \leftarrow \frac{R^2}{\epsilon'} \log{T}\log{\frac{\log{T }}{\delta'}}$ where $\epsilon' = \frac{\epsilon}{d}$ and $\delta' = \frac{\delta}{d}$
		\STATE Initialize Binary Tree $\B$ and define $B_s$ and $\hat{\B}_s$ to be the exact and the noisy versions of the value at node labeled $s$.
		%\STATE Initialize $sum \leftarrow 0$
		%\STATE {\bf Segments}. For $i \in \{1, . . . , log T \}$, associate with each string $s \in \{0, 1\}^i$  the time segment $S$ of $2^{log T - i}$ time periods
%$\{s \circ 0^{logT- i},...s \circ 1^{logT - i}\}$. The segment begins in time $s\circ 0^{logT - i}$ and ends in time $s \circ 1^{logT - i}$
		%\STATE For each node (with label $s$ say) sample $\zeta_S \sim \mathcal{N}(0, \sigma^2)$
		\FOR{$\tau = 1$ to $T$} 
			\STATE $sum = sum + \uu_{\tau}$
			\STATE Let $s_{\tau}$ be the string representation of $\tau$ in binary.
			\STATE Create all nodes in the tree whose labels are $s$ such that $s_{\tau} = s\circ t$ and $t = 1^{c}$ for some $c < k$. 
			\STATE Initialize each of the nodes created with for $i\leq d$ $\bm{\zeta}_s(i) = \mathcal{N}(0,\sigma^2)$
			\STATE Update the value at each node $s$ created :\\$\hat{B}_s \leftarrow B_s + \bm{\zeta_s}$\\ $B_s \leftarrow B_s + B_{s\circ 0} + B_{s\circ 1}$
			\STATE Let $s_1, s_2,... ,s_{\log {T}}$ be the ${\log{T}}$ labels such that each $s_i$ is a prefix of $s_{\tau}$ \label{line:addNoise}
			\STATE {\bf Output:} $Sum_i = sum+\sum_{i=1}^{\log{T}}\hat{B_{s_i}} $
		\ENDFOR					
	\end{algorithmic}
	\label{Algo:partialSum}
\end{algorithm} 

\begin{thm}[Privacy] \label{PartialSumPrivacy}
Let $R \geq max_{i \leq T}\ltwo{\uu_i} $ and $ \sigma^2 = \frac{R^2}{\epsilon'} \log{T}\log{\frac{\log{T }}{\delta'}}$  where $\epsilon' = \frac{\epsilon}{d}$ and $\delta' = \frac{\delta}{d}$. Then the Private Partial Sum algorithm when run with the parameters $(\epsilon, \delta, R) $ outputs every partial sum with a random Gaussian error of  $\mathcal{N}(0, \sigma_{cum}^2)$ in every entry of the output vector where $\sigma_{cum} \leq \sigma\cdot \log{T}$  and enjoys $(\epsilon, \delta)$-differential privacy against a single intrusion.
\end{thm}



\begin{proof}
Line \ref{line:addNoise} of the algorithm adds at most $\log{T}$ vectors all of which have each of their entries chosen from an independent Gaussian distribution (noise)$ \mathcal{N}(0, \sigma^2)$. Since each of these random variables is independent, each entry in the output vector has a random Gaussian error of  $\mathcal{N}(0, \sigma_{cum}^2)$ where $\sigma_{cum} \leq \sigma\cdot \log{T}$.

If every entry of a vector of dimension $d$ is $(\frac{\epsilon}{d}, \frac{\delta}{d})$ differentially private then the vector itself is $(\epsilon, \delta)$ differentially private. Thus, without loss of generality we assume that $d =1 $ and proceed with the proof. 

To prove the differential privacy for any partial sum output by the algorithm, we show that at all times the values stored in the tree $B$ are differentially private. The partial sum returned by the algorithm at time $\tau$ is a function of the values stored at any of the existing nodes of the binary tree $B$ at $\tau$. The privacy guarantees for the partial sums then follows from the preservation of differential privacy under compositions. 

For the purpose of privacy guarantees, the Binary tree $\B$ can be seen as a vector of at most $2T-1$ values stored at its nodes. We refer to this vector as $\B$.
  Let $B_{s_1}, B_{s_2}, ..., $ be an arbitrary ordering of the nodes of $B$

 Let $\u$ and $\u'$ be two sets of inputs to the algorithm differing in exactly one entry, say at time $\tau$. Let the binary tree vectors produced in the two runs of the algorithm be $\B(\u)$ and $\B(\u')$ respectively. Consider          

\begin{claim}\label{claimBTree}
Suppose for any node $B_s$ at time $\tau$, $\Pr_{B^*_{s}} [e^{-\frac{\epsilon}{\log{T}} }  \leq \frac{ \Pr [ B_{s}(\u) = B^*_{s}]}  { \Pr[ B_{s_1}(\u') = B^*_{s}]}  \leq e^{\frac{\epsilon}{\log{T}} } ] \geq 1 - \frac{\delta}{\log{T}} $. Then $\B$ is $(\epsilon, \delta)$ differentially private at time $\tau$. 
\end{claim}
We first show how the claim implies the theorem. We then prove the claim and complete the proof.
Now, $$\frac{\Pr [ \B(\u) \in  S]}{\Pr [\B(\u') \in S]} =  \frac{\int_{\B^* \in S}\Pr [ \B(\u) = \B^*]}{\int_{\B^* \in S} \Pr [\B(\u') \in \B^*]} $$
\begin{align*}
\frac{ \Pr [ \B(\u) = \B^*]}  { \Pr [\B(\u') \in \B^*]}  &=  \frac{ \Pr [ B_{s_1}(\u) = B^*_{s_1}]} { Prob B_{s_1}(\u') = B^*_{s_1}]}  \frac{ \Pr [ B_{s_2}(\u) = B^*_{s_2} |  B_{s_1}(\u) = B^*_{s_1}]}  { Prob B_{s_1}(\u') = B^*_{s_1}   |  B_{s_1}(\u') = B^*_{s_1}] }\cdots\\
&= \frac{ \Pr [ B_{s_1}(\u) = B^*_{s_1}]} { \Pr[ B_{s_1}(\u') = B^*_{s_1}]}  \frac{ \Pr [ B_{s_2}(\u) = B^*_{s_2}]}  { \Pr[ B_{s_1}(\u') = B^*_{s_1} ] }\cdots\\
&\text{(follows from the independence of every noise vector added)}
\end{align*}
 Since $\u$ and $\u'$ differ in exactly one entry, $B(\u)$ and $B(\u')$ can differ in at most $\log{T}$ nodes. Thus at most $\log{T}$ ratios in the above product can be different from $1$. Thus by using the Claim and a Union Bound over the at most $\log{T}$ nodes which have differing values in $B(\u)$ and $B(\u')$, we have 
$$\Pr [e^{-\epsilon} \leq \frac{ \Pr [ \B(\u) = \B^*]} { \Pr [\B(\u') \in \B^*]}  \leq e^{\epsilon}] \geq 1 - \sum \frac{\delta}{\log{T}} = 1 - \delta$$
Thus , 
$$ \frac{ Pr [ \B(\u) = \B^*]}  { \Pr [\B(\u') = \B^*]}  \leq e^{-\epsilon } ( 1- \delta) + \delta \leq e^{\epsilon} + \delta $$ 
We now show the validity of the claim and complete the proof.

\begin{proof}[Proof of Claim \ref{claimBTree}]
Let $\Delta = B_s(\u) - B_s(\u')$
\begin{align*}
 \frac{ \Pr [ B_{s}(\u) = B^*_{s}]}  { \Pr [B_{s}(\u') = B^*_{s}]} &= \frac { \exp{\frac{\ltwo{B^*_s - B_s(\u)  }^2)}{2\sigma_{cum}^2}}}{ \exp{\frac{\ltwo{B^*_s - B_s(\u')  }^2)}{2\sigma_{cum}^2}} }
= \exp{ \frac{ \ltwo{\Delta }^2  - 2\Delta ^T (B(\u')- B^*_s) }{2\sigma_{cum}^2} },\\
&\leq \exp{ \frac{ \ltwo{\Delta }^2  + 2\Delta ^T (B(\u')- B^*_s) }{2\sigma_{cum}^2} } ,
\end{align*}
Now, $\Delta^T(B(\u')- B^*_s)$ follows $\mathcal{N}(0,\ltwo{\Delta}^2\sigma_{cum}^2 )$.  Let $\mathcal{G} =\{B^*_s | \ltwo{ \Delta^T(B(\u') - B^*_s)} \leq \ltwo{\Delta} \sigma t\}$. 

If a random variable $V\sim\mathcal{N}(0,1)$, then for all $t>1$, one has $\Pr[|V|>t]\leq e^{-t^2/2}$ ( Mill's inequality ). Thus, 
  $$\Pr [\ltwo{ \Delta^T(B(\u') - B^*_s)} \leq\ltwo{\Delta} \sigma t] \leq \exp(\frac{-t^2}{2})$$
Setting $ t= 2\sqrt{   \ln{   \frac{2\log{T}}{\delta}}        }$, we have,  with probability $1 -\frac{ \delta}{2\log{T}}$ \\
\begin{equation} \Pr [ B_{s}(\u) = B^*_{s}] \leq \exp{\frac{\epsilon}{\log{T}}}   \Pr [B_{s}(\u') = B^*_{s}]   \label{eq:2} \end{equation}

Similarly, with probability at least $1 - \frac{\delta}{2\log{T}}$ \begin{equation} \Pr [ B_{s}(\u') = B^*_{s}] \leq \exp{\frac{\epsilon}{\log{T}}}   \Pr [B_{s}(\u) = B^*_{s}]   \label{eq:1} \end{equation}
 
Using union bound with equations \eqref{eq:2} and \eqref{eq:1}, we have the claim. 
\end{proof}


Thus the proof of the theorem is now complete.
\end{proof} 
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "nips2011"
%%% End: 

